Waveform Signal Entropy and Compression Study of Whole-Building Energy Datasets

Electrical energy consumption has been an ongoing research area since the coming of smart homes and Internet of Things devices. Consumption characteristics and usages profiles are directly influenced by building occupants and their interaction with electrical appliances. Extracted information from these data can be used to conserve energy and increase user comfort levels. Data analysis together with machine learning models can be utilized to extract valuable information for the benefit of occupants themselves, power plants, and grid operators. Public energy datasets provide a scientific foundation to develop and benchmark these algorithms and techniques. With datasets exceeding tens of terabytes, we present a novel study of five whole-building energy datasets with high sampling rates, their signal entropy, and how a well-calibrated measurement can have a significant effect on the overall storage requirements. We show that some datasets do not fully utilize the available measurement precision, therefore leaving potential accuracy and space savings untapped. We benchmark a comprehensive list of 365 file formats, transparent data transformations, and lossless compression algorithms. The primary goal is to reduce the overall dataset size while maintaining an easy-to-use file format and access API. We show that with careful selection of file format and encoding scheme, we can reduce the size of some datasets by up to 73%.

==> 00-keywords.tex <==
% !TEX root = energy-data-compression-paper.tex

%
% The code below should be generated by the tool at
% http://dl.acm.org/ccs.cfm
% Please copy and paste the code instead of the example below.
%
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10010583.10010662.10010668.10010669</concept_id>
<concept_desc>Hardware~Energy metering</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10002951.10002952.10002971.10003451.10002975</concept_id>
<concept_desc>Information systems~Data compression</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10002951.10003317.10003318.10003323</concept_id>
<concept_desc>Information systems~Data encoding and canonicalization</concept_desc>
<concept_significance>300</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Hardware~Energy metering}
\ccsdesc[300]{Information systems~Data compression}
\ccsdesc[300]{Information systems~Data encoding and canonicalization}

\keywords{Energy dataset, high sampling rate, non-intrusive load monitoring, file format, waveform compression, electricity aggregate}


==> results/file_format_longtable.tex <==
\tiny \begin{longtable}{lc|lc}
\caption{REDD: Data representation benchmark \numberOfDataRepresentations{} formats and data transformations. Raw input data size was \SI{1.4}{\gibi\byte} from 42 files.} \\
\textbf{Name} & \textbf{Compression Ratio} & \textbf{Name} & \textbf{Compression Ratio} \\ \hline \endhead
bzip2 LEB128S-delta-row & 51.7 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'snappy') all-column-chunk & 71.8 \% \\
Zarr BZ2 (Delta(dtype='<i4'),) & 52.3 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zlib') all-column-chunk & 71.8 \% \\
Zarr LZMA (Delta(dtype='<i4'),) & 53.8 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'snappy') all-column-chunk & 71.8 \% \\
FLAC PCM-24 & 53.8 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'snappy') all-column-chunk & 71.8 \% \\
Zarr Blosc-zstd shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i4'),) & 54.5 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'snappy') all-column-chunk & 71.8 \% \\
ALAC PCM-24 & 54.6 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zlib') all-column-chunk & 71.8 \% \\
HDF5 shuffle zstd all-column-chunk & 55.1 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zlib') all-column-chunk & 71.8 \% \\
LZMA-alone LEB128S-delta-row & 55.1 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'snappy') all-column-chunk & 71.8 \% \\
LZMA-xz LEB128S-delta-row & 55.1 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zlib') all-column-chunk & 71.8 \% \\
HDF5 shuffle zstd individual-dsets & 55.1 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zlib') all-column-chunk & 71.8 \% \\
HDF5 no-shuffle MAFISC-LZMA individual-dsets & 55.2 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'snappy') all-column-chunk & 71.8 \% \\
Zarr Blosc-zstd shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i4'),) & 55.8 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zlib') all-column-chunk & 71.8 \% \\
WavPack PCM-24 & 55.9 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zlib') all-column-chunk & 71.8 \% \\
LZMA raw-column DELTA distance-3 & 57.1 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'snappy') all-column-chunk & 71.8 \% \\
zstd-22 LEB128S-delta-row & 58.2 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4hc') all-column-chunk & 71.9 \% \\
Zarr Blosc-zstd shuffle=BITSHUFFLE, blocksize=0) & 58.5 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4hc') all-column-chunk & 71.9 \% \\
Zarr Blosc(cname='zlib', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i4'),) & 58.6 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4hc') all-column-chunk & 71.9 \% \\
Zarr Blosc-zstd shuffle=SHUFFLE, blocksize=0) & 59.1 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4hc') all-column-chunk & 71.9 \% \\
LZMA-alone raw-column & 59.7 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4hc') all-column-chunk & 71.9 \% \\
LZMA-xz raw-column & 59.7 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4hc') all-column-chunk & 71.9 \% \\
Zarr Blosc(cname='zlib', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i4'),) & 59.7 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4hc') all-column-chunk & 71.9 \% \\
Zarr Blosc(cname='lz4hc', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i4'),) & 60.0 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4hc') all-column-chunk & 71.9 \% \\
bzip2 LEB128S-delta-column & 60.3 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4hc') all-column-chunk & 71.9 \% \\
Zarr Blosc(cname='zlib', shuffle=BITSHUFFLE, blocksize=0) & 60.7 \% & zstd-22 LEB128S-row & 71.9 \% \\
Zarr LZMA & 60.7 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zlib') individual-dsets & 72.0 \% \\
HDF5 shuffle gzip all-column-chunk & 60.8 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zlib') individual-dsets & 72.0 \% \\
HDF5 shuffle gzip individual-dsets & 60.8 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zlib') individual-dsets & 72.0 \% \\
LZMA-alone LEB128S-row & 60.9 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zlib') individual-dsets & 72.0 \% \\
LZMA-xz LEB128S-row & 60.9 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zlib') individual-dsets & 72.0 \% \\
LZMA-alone LEB128S-delta-column & 61.2 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zlib') individual-dsets & 72.0 \% \\
LZMA-xz LEB128S-delta-column & 61.2 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zlib') individual-dsets & 72.0 \% \\
HDF5 shuffle MAFISC-LZMA individual-dsets & 61.3 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zlib') individual-dsets & 72.0 \% \\
Zarr Blosc(cname='zlib', shuffle=SHUFFLE, blocksize=0) & 61.7 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zlib') individual-dsets & 72.0 \% \\
HDF5 shuffle zstd all-row-chunk & 62.1 \% & HDF5 shuffle MAFISC-LZMA all-row-chunk & 72.1 \% \\
Zarr Blosc(cname='lz4hc', shuffle=BITSHUFFLE, blocksize=0) & 62.8 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4hc') individual-dsets & 72.2 \% \\
bzip2 raw-column & 62.9 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4hc') individual-dsets & 72.2 \% \\
Zarr Blosc(cname='lz4', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i4'),) & 63.0 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4hc') individual-dsets & 72.2 \% \\
zstd-22 LEB128S-delta-column & 63.1 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4hc') individual-dsets & 72.2 \% \\
HDF5 shuffle MAFISC-LZMA all-column-chunk & 63.5 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4hc') individual-dsets & 72.2 \% \\
Zarr Blosc(cname='lz4hc', shuffle=SHUFFLE, blocksize=0) & 63.8 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4hc') individual-dsets & 72.2 \% \\
HDF5 no-shuffle MAFISC-LZMA all-column-chunk & 63.8 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4hc') individual-dsets & 72.2 \% \\
bzip2 LEB128S-row & 64.4 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4hc') individual-dsets & 72.2 \% \\
LZMA-alone raw-row & 65.1 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4hc') individual-dsets & 72.2 \% \\
LZMA-xz raw-row & 65.2 \% & HDF5 shuffle bitshuffle-lz4 all-column-chunk & 72.4 \% \\
LZMA LEB128S-delta-row DELTA distance-1 & 65.4 \% & HDF5 shuffle bitshuffle-lz4 individual-dsets & 72.4 \% \\
ZLIB LEB128S-delta-row & 65.7 \% & Zarr Blosc(cname='zlib', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i4'),) & 72.5 \% \\
HDF5 shuffle gzip all-row-chunk & 66.7 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'snappy') individual-dsets & 72.5 \% \\
LZMA LEB128S-delta-row DELTA distance-3 & 66.8 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'snappy') individual-dsets & 72.5 \% \\
Zarr Blosc(cname='lz4', shuffle=BITSHUFFLE, blocksize=0) & 66.9 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'snappy') individual-dsets & 72.5 \% \\
Zarr BZ2 & 66.9 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'snappy') individual-dsets & 72.5 \% \\
Zarr Blosc(cname='lz4hc', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i4'),) & 67.4 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'snappy') individual-dsets & 72.5 \% \\
ZLIB LEB128S-delta-column & 67.9 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'snappy') individual-dsets & 72.5 \% \\
Zarr Blosc(cname='snappy', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i4'),) & 67.9 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'snappy') individual-dsets & 72.5 \% \\
HDF5 no-shuffle ('SZIP', 'nn', 8) all-column-chunk & 68.0 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'snappy') individual-dsets & 72.5 \% \\
HDF5 no-shuffle ('SZIP', 'nn', 8) individual-dsets & 68.0 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'snappy') individual-dsets & 72.5 \% \\
Zarr Blosc-zstd shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i4'),) & 68.1 \% & HDF5 no-shuffle ('SZIP', 'nn', 32) all-column-chunk & 72.8 \% \\
LZMA raw-row DELTA distance-3 & 68.2 \% & HDF5 no-shuffle ('SZIP', 'nn', 32) individual-dsets & 72.8 \% \\
HDF5 no-shuffle MAFISC-LZMA all-row-chunk & 68.7 \% & LZMA LEB128S-row DELTA distance-3 & 72.9 \% \\
Zarr Blosc(cname='snappy', shuffle=BITSHUFFLE, blocksize=0) & 68.8 \% & LZMA LEB128S-delta-column DELTA distance-2 & 73.6 \% \\
LZMA-alone LEB128S-column & 69.0 \% & HDF5 no-shuffle bitshuffle-lz4 all-column-chunk & 74.1 \% \\
LZMA-xz LEB128S-column & 69.0 \% & HDF5 no-shuffle bitshuffle-lz4 individual-dsets & 74.1 \% \\
HDF5 no-shuffle ('SZIP', 'nn', 16) all-column-chunk & 69.0 \% & LZMA LEB128S-delta-column DELTA distance-4 & 74.6 \% \\
HDF5 no-shuffle ('SZIP', 'nn', 16) individual-dsets & 69.1 \% & LZMA LEB128S-delta-column DELTA distance-3 & 74.7 \% \\
Zarr Blosc(cname='lz4', shuffle=SHUFFLE, blocksize=0) & 69.3 \% & LZMA raw-column DELTA distance-1 & 74.9 \% \\
HDF5 shuffle lzf all-column-chunk & 69.7 \% & HDF5 no-shuffle ('SZIP', 'nn', 2) all-column-chunk & 75.8 \% \\
HDF5 shuffle lzf individual-dsets & 69.7 \% & HDF5 no-shuffle ('SZIP', 'nn', 2) individual-dsets & 75.8 \% \\
zstd-22 raw-column & 69.7 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zstd') all-row-chunk & 75.9 \% \\
HDF5 no-shuffle ('SZIP', 'nn', 4) all-column-chunk & 69.9 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zstd') all-row-chunk & 75.9 \% \\
HDF5 no-shuffle ('SZIP', 'nn', 4) individual-dsets & 69.9 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zstd') all-row-chunk & 75.9 \% \\
LZMA LEB128S-delta-row DELTA distance-2 & 70.0 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zstd') all-row-chunk & 75.9 \% \\
Zarr Blosc(cname='snappy', shuffle=SHUFFLE, blocksize=0) & 70.3 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zstd') all-row-chunk & 75.9 \% \\
HDF5 no-shuffle zstd all-column-chunk & 70.6 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zstd') all-row-chunk & 75.9 \% \\
HDF5 no-shuffle ('SZIP', 'nn', 24) all-column-chunk & 70.8 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zstd') all-row-chunk & 75.9 \% \\
HDF5 no-shuffle ('SZIP', 'nn', 24) individual-dsets & 70.8 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zstd') all-row-chunk & 75.9 \% \\
HDF5 no-shuffle zstd individual-dsets & 71.1 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zstd') all-row-chunk & 75.9 \% \\
LZMA LEB128S-delta-row DELTA distance-4 & 71.1 \% & Zarr Blosc(cname='blosclz', shuffle=SHUFFLE, blocksize=0) & 76.0 \% \\
LZMA LEB128S-delta-column DELTA distance-1 & 71.2 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'snappy') all-row-chunk & 76.2 \% \\
Zarr Zlib(level=9) (Delta(dtype='<i4'),) & 71.5 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zlib') all-row-chunk & 76.2 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zstd') all-column-chunk & 71.7 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'snappy') all-row-chunk & 76.2 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zstd') all-column-chunk & 71.7 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'snappy') all-row-chunk & 76.2 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zstd') all-column-chunk & 71.7 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'snappy') all-row-chunk & 76.2 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zstd') all-column-chunk & 71.7 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zlib') all-row-chunk & 76.2 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zstd') all-column-chunk & 71.7 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zlib') all-row-chunk & 76.2 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zstd') all-column-chunk & 71.7 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'snappy') all-row-chunk & 76.2 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zstd') all-column-chunk & 71.7 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zlib') all-row-chunk & 76.2 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zstd') all-column-chunk & 71.7 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zlib') all-row-chunk & 76.2 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zstd') all-column-chunk & 71.7 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'snappy') all-row-chunk & 76.2 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zstd') individual-dsets & 71.7 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zlib') all-row-chunk & 76.2 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zstd') individual-dsets & 71.7 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zlib') all-row-chunk & 76.2 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zstd') individual-dsets & 71.7 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zlib') all-row-chunk & 76.2 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zstd') individual-dsets & 71.7 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'snappy') all-row-chunk & 76.2 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zstd') individual-dsets & 71.7 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'snappy') all-row-chunk & 76.2 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zstd') individual-dsets & 71.7 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'snappy') all-row-chunk & 76.2 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zstd') individual-dsets & 71.7 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zlib') all-row-chunk & 76.2 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zstd') individual-dsets & 71.7 \% & bzip2 raw-row & 76.4 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zstd') individual-dsets & 71.7 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4hc') all-row-chunk & 76.7 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zlib') all-column-chunk & 71.8 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4hc') all-row-chunk & 76.7 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zlib') all-column-chunk & 71.8 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4hc') all-row-chunk & 76.7 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'snappy') all-column-chunk & 71.8 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4hc') all-row-chunk & 76.7 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'snappy') all-column-chunk & 71.8 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4hc') all-row-chunk & 76.7 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4hc') all-row-chunk & 76.7 \% & HDF5 shuffle ('SZIP', 'ec', 4) all-column-chunk & 116.7 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4hc') all-row-chunk & 76.7 \% & HDF5 shuffle ('SZIP', 'ec', 4) individual-dsets & 116.7 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4hc') all-row-chunk & 76.7 \% & HDF5 no-shuffle ('SZIP', 'nn', 4) all-row-chunk & 117.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4hc') all-row-chunk & 76.7 \% & HDF5 shuffle ('SZIP', 'nn', 24) all-row-chunk & 117.1 \% \\
zstd-22 raw-row & 76.8 \% & HDF5 shuffle ('SZIP', 'nn', 4) all-row-chunk & 117.8 \% \\
HDF5 no-shuffle zstd all-row-chunk & 77.6 \% & HDF5 shuffle ('SZIP', 'nn', 32) all-row-chunk & 117.8 \% \\
HDF5 shuffle lzf all-row-chunk & 77.6 \% & HDF5 shuffle ('SZIP', 'ec', 16) all-column-chunk & 119.2 \% \\
Zarr Blosc(cname='snappy', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i4'),) & 77.9 \% & HDF5 shuffle ('SZIP', 'ec', 16) individual-dsets & 119.2 \% \\
zstd-22 LEB128S-column & 78.3 \% & HDF5 no-shuffle lzf all-column-chunk & 119.9 \% \\
bzip2 LEB128S-column & 78.5 \% & HDF5 no-shuffle lzf individual-dsets & 119.9 \% \\
LZMA LEB128S-row DELTA distance-1 & 79.1 \% & Zarr Blosc(cname='lz4', shuffle=NOSHUFFLE, blocksize=0) & 120.3 \% \\
HDF5 shuffle bitshuffle-lz4 all-row-chunk & 80.5 \% & Zarr Blosc(cname='blosclz', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i4'),) & 122.4 \% \\
ZLIB raw-column & 81.3 \% & HDF5 no-shuffle ('SZIP', 'ec', 32) all-row-chunk & 122.6 \% \\
Zarr Blosc-zstd shuffle=NOSHUFFLE, blocksize=0) & 82.0 \% & HDF5 no-shuffle ('SZIP', 'ec', 24) all-row-chunk & 122.6 \% \\
Zarr Blosc(cname='lz4', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i4'),) & 82.4 \% & HDF5 no-shuffle ('SZIP', 'ec', 2) all-column-chunk & 122.7 \% \\
HDF5 no-shuffle bitshuffle-lz4 all-row-chunk & 82.5 \% & HDF5 no-shuffle ('SZIP', 'ec', 2) individual-dsets & 122.7 \% \\
Zarr Blosc(cname='blosclz', shuffle=BITSHUFFLE, blocksize=0) & 82.7 \% & HDF5 no-shuffle ('SZIP', 'ec', 16) all-row-chunk & 123.0 \% \\
HDF5 shuffle ('SZIP', 'nn', 4) all-column-chunk & 83.3 \% & Zarr Blosc(cname='snappy', shuffle=NOSHUFFLE, blocksize=0) & 124.0 \% \\
HDF5 shuffle ('SZIP', 'nn', 4) individual-dsets & 83.3 \% & HDF5 shuffle ('SZIP', 'ec', 24) all-column-chunk & 124.0 \% \\
LZMA LEB128S-row DELTA distance-2 & 84.0 \% & HDF5 shuffle ('SZIP', 'ec', 24) individual-dsets & 124.0 \% \\
LZMA LEB128S-row DELTA distance-4 & 84.3 \% & HDF5 no-shuffle ('SZIP', 'ec', 8) all-row-chunk & 124.1 \% \\
ZLIB LEB128S-row & 84.6 \% & HDF5 shuffle ('SZIP', 'ec', 16) all-row-chunk & 124.3 \% \\
HDF5 shuffle ('SZIP', 'nn', 8) all-column-chunk & 85.0 \% & HDF5 shuffle ('SZIP', 'ec', 2) all-column-chunk & 124.6 \% \\
HDF5 shuffle ('SZIP', 'nn', 8) individual-dsets & 85.0 \% & HDF5 shuffle ('SZIP', 'ec', 2) individual-dsets & 124.6 \% \\
LZMA LEB128S-column DELTA distance-3 & 85.6 \% & HDF5 shuffle ('SZIP', 'ec', 8) all-row-chunk & 124.7 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4') all-column-chunk & 86.5 \% & HDF5 shuffle ('SZIP', 'ec', 24) all-row-chunk & 124.7 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4') all-column-chunk & 86.5 \% & HDF5 shuffle ('SZIP', 'ec', 32) all-row-chunk & 125.3 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4') all-column-chunk & 86.5 \% & HDF5 no-shuffle ('SZIP', 'ec', 4) all-row-chunk & 126.5 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4') all-column-chunk & 86.5 \% & HDF5 no-shuffle lzf all-row-chunk & 126.6 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4') all-column-chunk & 86.5 \% & HDF5 shuffle ('SZIP', 'ec', 4) all-row-chunk & 126.9 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4') all-column-chunk & 86.5 \% & HDF5 shuffle ('SZIP', 'ec', 32) all-column-chunk & 129.2 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4') all-column-chunk & 86.5 \% & HDF5 shuffle ('SZIP', 'ec', 32) individual-dsets & 129.3 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4') all-column-chunk & 86.5 \% & Zarr Blosc(cname='blosclz', shuffle=NOSHUFFLE, blocksize=0) & 130.7 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4') all-column-chunk & 86.5 \% & Zarr None & 133.3 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4') individual-dsets & 86.6 \% & Zarr None (Delta(dtype='<i4'),) & 133.3 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4') individual-dsets & 86.6 \% & HDF5 no-shuffle ('SZIP', 'nn', 2) all-row-chunk & 133.3 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4') individual-dsets & 86.6 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'blosclz') all-row-chunk & 133.3 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4') individual-dsets & 86.6 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'blosclz') all-row-chunk & 133.3 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4') individual-dsets & 86.6 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'blosclz') all-column-chunk & 133.3 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4') individual-dsets & 86.6 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'blosclz') all-column-chunk & 133.3 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4') individual-dsets & 86.6 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'blosclz') all-row-chunk & 133.3 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4') individual-dsets & 86.6 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'blosclz') all-row-chunk & 133.3 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4') individual-dsets & 86.6 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'blosclz') all-row-chunk & 133.3 \% \\
ZLIB raw-row & 87.3 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'blosclz') all-row-chunk & 133.3 \% \\
HDF5 shuffle ('SZIP', 'nn', 2) all-column-chunk & 87.4 \% & HDF5 shuffle ('SZIP', 'ec', 2) all-row-chunk & 133.3 \% \\
HDF5 shuffle ('SZIP', 'nn', 2) individual-dsets & 87.4 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'blosclz') all-column-chunk & 133.3 \% \\
LZMA raw-column DELTA distance-2 & 87.9 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'blosclz') all-row-chunk & 133.3 \% \\
LZMA LEB128S-column DELTA distance-1 & 88.9 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'blosclz') all-column-chunk & 133.3 \% \\
ZLIB LEB128S-column & 89.2 \% & HDF5 no-shuffle ('SZIP', 'ec', 2) all-row-chunk & 133.3 \% \\
LZMA raw-row DELTA distance-1 & 89.2 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'blosclz') all-column-chunk & 133.3 \% \\
Zarr Blosc(cname='blosclz', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i4'),) & 89.3 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'blosclz') all-column-chunk & 133.3 \% \\
HDF5 no-shuffle gzip all-column-chunk & 89.7 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'blosclz') all-row-chunk & 133.3 \% \\
HDF5 no-shuffle gzip individual-dsets & 89.8 \% & HDF5 shuffle ('SZIP', 'nn', 2) all-row-chunk & 133.3 \% \\
Zarr Zlib(level=9) & 90.0 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'blosclz') all-row-chunk & 133.3 \% \\
Zarr Blosc(cname='lz4hc', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i4'),) & 90.5 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'blosclz') all-column-chunk & 133.3 \% \\
Zarr Blosc(cname='zlib', shuffle=NOSHUFFLE, blocksize=0) & 90.9 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'blosclz') all-column-chunk & 133.3 \% \\
Zarr Blosc(cname='blosclz', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i4'),) & 91.2 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'blosclz') all-column-chunk & 133.3 \% \\
HDF5 shuffle ('SZIP', 'nn', 16) all-column-chunk & 92.2 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'blosclz') individual-dsets & 133.4 \% \\
HDF5 shuffle ('SZIP', 'nn', 16) individual-dsets & 92.2 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'blosclz') individual-dsets & 133.4 \% \\
LZMA LEB128S-column DELTA distance-4 & 94.5 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'blosclz') individual-dsets & 133.4 \% \\
LZMA LEB128S-column DELTA distance-2 & 95.1 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'blosclz') individual-dsets & 133.4 \% \\
LZMA raw-column DELTA distance-4 & 96.6 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'blosclz') individual-dsets & 133.4 \% \\
LZMA raw-row DELTA distance-2 & 97.5 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'blosclz') individual-dsets & 133.4 \% \\
HDF5 no-shuffle gzip all-row-chunk & 97.9 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'blosclz') individual-dsets & 133.4 \% \\
HDF5 shuffle ('SZIP', 'nn', 24) all-column-chunk & 98.0 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'blosclz') individual-dsets & 133.4 \% \\
HDF5 shuffle ('SZIP', 'nn', 24) individual-dsets & 98.0 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'blosclz') individual-dsets & 133.4 \% \\
LZMA raw-row DELTA distance-4 & 99.9 \%  \\
RAW-UNCOMPRESSED & 100.0 \%  \\
HDF5 shuffle ('SZIP', 'nn', 32) all-column-chunk & 103.9 \%  \\
HDF5 shuffle ('SZIP', 'nn', 32) individual-dsets & 103.9 \%  \\
Zarr Blosc(cname='snappy', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i4'),) & 107.3 \%  \\
Zarr Blosc(cname='lz4hc', shuffle=NOSHUFFLE, blocksize=0) & 107.5 \%  \\
Zarr Blosc(cname='lz4', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i4'),) & 108.7 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 16) all-column-chunk & 109.1 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 16) individual-dsets & 109.1 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 8) all-column-chunk & 109.7 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 8) individual-dsets & 109.7 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 24) all-column-chunk & 110.1 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 24) individual-dsets & 110.1 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 32) all-column-chunk & 111.5 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 32) individual-dsets & 111.5 \%  \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4') all-row-chunk & 113.5 \%  \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4') all-row-chunk & 113.5 \%  \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4') all-row-chunk & 113.5 \%  \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4') all-row-chunk & 113.5 \%  \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4') all-row-chunk & 113.5 \%  \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4') all-row-chunk & 113.5 \%  \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4') all-row-chunk & 113.5 \%  \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4') all-row-chunk & 113.5 \%  \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4') all-row-chunk & 113.5 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 4) all-column-chunk & 113.7 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 4) individual-dsets & 113.7 \%  \\
HDF5 no-shuffle ('SZIP', 'nn', 24) all-row-chunk & 113.7 \%  \\
HDF5 no-shuffle ('SZIP', 'nn', 16) all-row-chunk & 113.8 \%  \\
HDF5 no-shuffle ('SZIP', 'nn', 32) all-row-chunk & 114.0 \%  \\
HDF5 no-shuffle ('SZIP', 'nn', 8) all-row-chunk & 115.0 \%  \\
HDF5 shuffle ('SZIP', 'ec', 8) all-column-chunk & 115.2 \%  \\
HDF5 shuffle ('SZIP', 'ec', 8) individual-dsets & 115.2 \%  \\
HDF5 shuffle ('SZIP', 'nn', 8) all-row-chunk & 116.3 \%  \\
HDF5 shuffle ('SZIP', 'nn', 16) all-row-chunk & 116.5 \%  \\
\end{longtable}
\tiny \begin{longtable}{lc|lc}
\caption{BLUED: Data representation benchmark \numberOfDataRepresentations{} formats and data transformations. Raw input data size was \SI{41.1}{\gibi\byte} from 6430 files.} \\
\textbf{Name} & \textbf{Compression Ratio} & \textbf{Name} & \textbf{Compression Ratio} \\ \hline \endhead
bzip2 LEB128S-row & 27.0 \% & HDF5 shuffle bitshuffle-lz4 individual-dsets & 57.9 \% \\
bzip2 raw-column & 27.1 \% & HDF5 no-shuffle ('SZIP', 'nn', 4) all-column-chunk & 58.8 \% \\
bzip2 LEB128S-delta-row & 27.9 \% & HDF5 no-shuffle ('SZIP', 'nn', 4) individual-dsets & 58.9 \% \\
LZMA-alone raw-column & 28.6 \% & HDF5 shuffle MAFISC-LZMA all-row-chunk & 59.1 \% \\
LZMA-xz raw-column & 28.6 \% & HDF5 no-shuffle ('SZIP', 'nn', 8) all-column-chunk & 59.3 \% \\
LZMA raw-column DELTA distance-2 & 28.8 \% & HDF5 no-shuffle ('SZIP', 'nn', 8) individual-dsets & 59.4 \% \\
Zarr LZMA & 29.5 \% & Zarr Blosc(cname='zlib', shuffle=NOSHUFFLE, blocksize=0) & 59.4 \% \\
Zarr BZ2 (Delta(dtype='<i2'),) & 29.5 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zstd') individual-dsets & 60.0 \% \\
Zarr LZMA (Delta(dtype='<i2'),) & 29.6 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zstd') individual-dsets & 60.0 \% \\
LZMA-alone LEB128S-delta-row & 30.1 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zstd') individual-dsets & 60.0 \% \\
LZMA-xz LEB128S-delta-row & 30.1 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zstd') individual-dsets & 60.0 \% \\
Zarr BZ2 & 30.2 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zstd') individual-dsets & 60.0 \% \\
LZMA-alone LEB128S-row & 30.5 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zstd') individual-dsets & 60.0 \% \\
LZMA-xz LEB128S-row & 30.5 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zstd') individual-dsets & 60.0 \% \\
LZMA raw-column DELTA distance-4 & 30.5 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zstd') individual-dsets & 60.0 \% \\
bzip2 LEB128S-delta-column & 30.8 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zstd') individual-dsets & 60.0 \% \\
LZMA-alone raw-row & 31.4 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zlib') individual-dsets & 60.0 \% \\
LZMA-xz raw-row & 31.4 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zlib') individual-dsets & 60.0 \% \\
LZMA LEB128S-row DELTA distance-2 & 32.4 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'snappy') individual-dsets & 60.0 \% \\
FLAC PCM-16 & 32.8 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'snappy') individual-dsets & 60.0 \% \\
ALAC PCM-16 & 33.8 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zlib') individual-dsets & 60.0 \% \\
zstd-22 LEB128S-delta-row & 34.0 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'snappy') individual-dsets & 60.0 \% \\
LZMA-alone LEB128S-delta-column & 34.5 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'snappy') individual-dsets & 60.0 \% \\
LZMA-xz LEB128S-delta-column & 34.5 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'snappy') individual-dsets & 60.0 \% \\
LZMA LEB128S-row DELTA distance-4 & 35.0 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'snappy') individual-dsets & 60.0 \% \\
LZMA LEB128S-delta-row DELTA distance-1 & 35.0 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'snappy') individual-dsets & 60.0 \% \\
WavPack PCM-16 & 35.2 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zlib') individual-dsets & 60.0 \% \\
LZMA LEB128S-delta-row DELTA distance-2 & 35.6 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zlib') individual-dsets & 60.0 \% \\
LZMA raw-row DELTA distance-2 & 35.9 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zlib') individual-dsets & 60.0 \% \\
HDF5 no-shuffle MAFISC-LZMA individual-dsets & 36.0 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zlib') individual-dsets & 60.0 \% \\
LZMA-alone LEB128S-column & 36.1 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zlib') individual-dsets & 60.0 \% \\
LZMA-xz LEB128S-column & 36.1 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'snappy') individual-dsets & 60.0 \% \\
LZMA raw-row DELTA distance-4 & 36.2 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zlib') individual-dsets & 60.0 \% \\
LZMA raw-column DELTA distance-1 & 36.6 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'snappy') individual-dsets & 60.0 \% \\
HDF5 shuffle zstd all-column-chunk & 37.3 \% & LZMA LEB128S-column DELTA distance-3 & 60.1 \% \\
LZMA LEB128S-delta-row DELTA distance-4 & 37.3 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zstd') all-column-chunk & 60.2 \% \\
HDF5 shuffle zstd individual-dsets & 37.4 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zstd') all-column-chunk & 60.2 \% \\
zstd-22 LEB128S-delta-column & 38.2 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zstd') all-column-chunk & 60.2 \% \\
Zarr Blosc-zstd shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 38.3 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zstd') all-column-chunk & 60.2 \% \\
Zarr Blosc-zstd shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 38.3 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zstd') all-column-chunk & 60.2 \% \\
LZMA LEB128S-row DELTA distance-1 & 38.6 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zstd') all-column-chunk & 60.2 \% \\
ZLIB LEB128S-delta-row & 38.9 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zstd') all-column-chunk & 60.2 \% \\
Zarr Blosc(cname='zlib', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 39.4 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zstd') all-column-chunk & 60.2 \% \\
Zarr Blosc-zstd shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 39.6 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zstd') all-column-chunk & 60.2 \% \\
zstd-22 LEB128S-row & 39.6 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zlib') all-column-chunk & 60.2 \% \\
zstd-22 raw-column & 40.1 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zlib') all-column-chunk & 60.2 \% \\
HDF5 no-shuffle zstd all-column-chunk & 40.1 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zlib') all-column-chunk & 60.2 \% \\
HDF5 no-shuffle zstd individual-dsets & 40.1 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zlib') all-column-chunk & 60.2 \% \\
Zarr Blosc-zstd shuffle=SHUFFLE, blocksize=0) & 40.4 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zlib') all-column-chunk & 60.2 \% \\
LZMA LEB128S-delta-row DELTA distance-3 & 40.8 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zlib') all-column-chunk & 60.2 \% \\
Zarr Blosc(cname='zlib', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 40.9 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zlib') all-column-chunk & 60.2 \% \\
Zarr Blosc(cname='zlib', shuffle=BITSHUFFLE, blocksize=0) & 41.0 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zlib') all-column-chunk & 60.2 \% \\
LZMA LEB128S-delta-column DELTA distance-4 & 41.3 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zlib') all-column-chunk & 60.2 \% \\
bzip2 LEB128S-column & 41.8 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'snappy') all-column-chunk & 60.5 \% \\
LZMA LEB128S-delta-column DELTA distance-1 & 42.1 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'snappy') all-column-chunk & 60.5 \% \\
bzip2 raw-row & 42.7 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'snappy') all-column-chunk & 60.5 \% \\
HDF5 no-shuffle MAFISC-LZMA all-column-chunk & 42.8 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'snappy') all-column-chunk & 60.5 \% \\
LZMA LEB128S-delta-column DELTA distance-2 & 42.9 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'snappy') all-column-chunk & 60.5 \% \\
Zarr Blosc(cname='lz4hc', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 43.2 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'snappy') all-column-chunk & 60.5 \% \\
HDF5 shuffle gzip all-column-chunk & 43.5 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'snappy') all-column-chunk & 60.5 \% \\
HDF5 shuffle gzip individual-dsets & 43.6 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'snappy') all-column-chunk & 60.5 \% \\
Zarr Zlib(level=9) (Delta(dtype='<i2'),) & 43.7 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'snappy') all-column-chunk & 60.5 \% \\
Zarr Blosc(cname='zlib', shuffle=SHUFFLE, blocksize=0) & 43.7 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4hc') all-column-chunk & 61.4 \% \\
Zarr Blosc-zstd shuffle=BITSHUFFLE, blocksize=0) & 44.4 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4hc') all-column-chunk & 61.4 \% \\
HDF5 shuffle MAFISC-LZMA individual-dsets & 45.0 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4hc') all-column-chunk & 61.4 \% \\
Zarr Blosc(cname='zlib', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 45.4 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4hc') all-column-chunk & 61.4 \% \\
Zarr Blosc(cname='lz4hc', shuffle=BITSHUFFLE, blocksize=0) & 45.4 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4hc') all-column-chunk & 61.4 \% \\
HDF5 no-shuffle zstd all-row-chunk & 45.5 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4hc') all-column-chunk & 61.4 \% \\
ZLIB LEB128S-delta-column & 45.6 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4hc') all-column-chunk & 61.4 \% \\
Zarr Blosc-zstd shuffle=NOSHUFFLE, blocksize=0) & 46.3 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4hc') all-column-chunk & 61.4 \% \\
Zarr Blosc(cname='lz4hc', shuffle=SHUFFLE, blocksize=0) & 46.7 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4hc') all-column-chunk & 61.4 \% \\
Zarr Blosc(cname='lz4', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 46.9 \% & Zarr Blosc(cname='blosclz', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 61.7 \% \\
LZMA raw-row DELTA distance-1 & 47.0 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4hc') individual-dsets & 61.9 \% \\
LZMA LEB128S-delta-column DELTA distance-3 & 47.1 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4hc') individual-dsets & 61.9 \% \\
HDF5 shuffle zstd all-row-chunk & 47.1 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4hc') individual-dsets & 61.9 \% \\
HDF5 shuffle MAFISC-LZMA all-column-chunk & 47.9 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4hc') individual-dsets & 61.9 \% \\
zstd-22 raw-row & 48.5 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4hc') individual-dsets & 61.9 \% \\
LZMA raw-column DELTA distance-3 & 48.7 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4hc') individual-dsets & 61.9 \% \\
LZMA LEB128S-row DELTA distance-3 & 49.5 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4hc') individual-dsets & 61.9 \% \\
Zarr Blosc(cname='lz4hc', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 49.7 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4hc') individual-dsets & 61.9 \% \\
zstd-22 LEB128S-column & 49.7 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4hc') individual-dsets & 61.9 \% \\
Zarr Blosc(cname='lz4', shuffle=BITSHUFFLE, blocksize=0) & 49.8 \% & LZMA raw-row DELTA distance-3 & 62.4 \% \\
LZMA LEB128S-column DELTA distance-2 & 50.4 \% & Zarr Blosc(cname='lz4', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 62.8 \% \\
HDF5 shuffle gzip all-row-chunk & 51.0 \% & HDF5 no-shuffle ('SZIP', 'nn', 2) all-column-chunk & 63.7 \% \\
Zarr Blosc(cname='blosclz', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 51.1 \% & HDF5 no-shuffle ('SZIP', 'nn', 2) individual-dsets & 63.8 \% \\
Zarr Blosc(cname='lz4', shuffle=SHUFFLE, blocksize=0) & 52.6 \% & HDF5 shuffle lzf all-row-chunk & 64.3 \% \\
LZMA LEB128S-column DELTA distance-1 & 54.2 \% & HDF5 no-shuffle ('SZIP', 'nn', 16) all-column-chunk & 65.2 \% \\
HDF5 no-shuffle MAFISC-LZMA all-row-chunk & 54.3 \% & HDF5 no-shuffle ('SZIP', 'nn', 16) individual-dsets & 65.3 \% \\
Zarr Blosc(cname='blosclz', shuffle=BITSHUFFLE, blocksize=0) & 54.5 \% & HDF5 no-shuffle gzip all-column-chunk & 65.5 \% \\
LZMA LEB128S-column DELTA distance-4 & 55.1 \% & HDF5 no-shuffle gzip individual-dsets & 65.5 \% \\
Zarr Blosc(cname='blosclz', shuffle=SHUFFLE, blocksize=0) & 55.2 \% & ZLIB raw-row & 66.8 \% \\
Zarr Blosc(cname='lz4hc', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 55.7 \% & ZLIB LEB128S-column & 67.1 \% \\
ZLIB LEB128S-row & 55.9 \% & Zarr Blosc(cname='lz4hc', shuffle=NOSHUFFLE, blocksize=0) & 67.5 \% \\
ZLIB raw-column & 56.8 \% & Zarr Blosc(cname='snappy', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 67.8 \% \\
HDF5 no-shuffle bitshuffle-lz4 all-column-chunk & 56.9 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zstd') all-row-chunk & 68.1 \% \\
HDF5 no-shuffle bitshuffle-lz4 individual-dsets & 57.0 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zstd') all-row-chunk & 68.1 \% \\
Zarr Zlib(level=9) & 57.3 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zstd') all-row-chunk & 68.1 \% \\
HDF5 shuffle lzf all-column-chunk & 57.8 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zstd') all-row-chunk & 68.1 \% \\
HDF5 shuffle bitshuffle-lz4 all-column-chunk & 57.8 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zstd') all-row-chunk & 68.1 \% \\
HDF5 shuffle lzf individual-dsets & 57.8 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zstd') all-row-chunk & 68.1 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zstd') all-row-chunk & 68.1 \% & HDF5 no-shuffle ('SZIP', 'ec', 32) individual-dsets & 153.1 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zstd') all-row-chunk & 68.1 \% & HDF5 shuffle ('SZIP', 'ec', 4) all-column-chunk & 155.3 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zstd') all-row-chunk & 68.1 \% & HDF5 shuffle ('SZIP', 'ec', 4) individual-dsets & 155.3 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zlib') all-row-chunk & 68.4 \% & HDF5 shuffle ('SZIP', 'ec', 8) all-column-chunk & 158.3 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zlib') all-row-chunk & 68.4 \% & HDF5 shuffle ('SZIP', 'ec', 8) individual-dsets & 158.4 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zlib') all-row-chunk & 68.4 \% & HDF5 no-shuffle ('SZIP', 'ec', 2) all-column-chunk & 158.4 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zlib') all-row-chunk & 68.4 \% & HDF5 no-shuffle ('SZIP', 'ec', 2) individual-dsets & 158.5 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zlib') all-row-chunk & 68.4 \% & HDF5 shuffle ('SZIP', 'ec', 2) all-column-chunk & 163.4 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zlib') all-row-chunk & 68.4 \% & HDF5 shuffle ('SZIP', 'ec', 2) individual-dsets & 163.5 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zlib') all-row-chunk & 68.4 \% & HDF5 shuffle ('SZIP', 'ec', 16) all-column-chunk & 174.3 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zlib') all-row-chunk & 68.4 \% & HDF5 shuffle ('SZIP', 'ec', 16) individual-dsets & 174.4 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zlib') all-row-chunk & 68.4 \% & HDF5 shuffle ('SZIP', 'ec', 24) all-column-chunk & 192.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'snappy') all-row-chunk & 68.4 \% & HDF5 shuffle ('SZIP', 'ec', 24) individual-dsets & 192.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'snappy') all-row-chunk & 68.4 \% & HDF5 no-shuffle ('SZIP', 'nn', 16) all-row-chunk & 198.6 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'snappy') all-row-chunk & 68.4 \% & HDF5 no-shuffle ('SZIP', 'nn', 8) all-row-chunk & 198.9 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'snappy') all-row-chunk & 68.4 \% & HDF5 no-shuffle ('SZIP', 'nn', 24) all-row-chunk & 198.9 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'snappy') all-row-chunk & 68.4 \% & HDF5 no-shuffle ('SZIP', 'nn', 32) all-row-chunk & 199.4 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'snappy') all-row-chunk & 68.4 \% & HDF5 no-shuffle ('SZIP', 'ec', 24) all-row-chunk & 199.5 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'snappy') all-row-chunk & 68.4 \% & HDF5 no-shuffle ('SZIP', 'ec', 16) all-row-chunk & 199.6 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'snappy') all-row-chunk & 68.4 \% & HDF5 no-shuffle ('SZIP', 'ec', 32) all-row-chunk & 199.7 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'snappy') all-row-chunk & 68.4 \% & HDF5 no-shuffle ('SZIP', 'nn', 4) all-row-chunk & 199.9 \% \\
Zarr Blosc(cname='snappy', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 68.5 \% & HDF5 shuffle ('SZIP', 'nn', 8) all-row-chunk & 199.9 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4hc') all-row-chunk & 68.8 \% & HDF5 shuffle ('SZIP', 'nn', 4) all-row-chunk & 199.9 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4hc') all-row-chunk & 68.8 \% & HDF5 no-shuffle ('SZIP', 'ec', 8) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4hc') all-row-chunk & 68.8 \% & HDF5 shuffle ('SZIP', 'nn', 16) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4hc') all-row-chunk & 68.8 \% & HDF5 shuffle ('SZIP', 'ec', 8) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4hc') all-row-chunk & 68.8 \% & HDF5 shuffle ('SZIP', 'ec', 16) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4hc') all-row-chunk & 68.8 \% & HDF5 shuffle ('SZIP', 'ec', 24) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4hc') all-row-chunk & 68.8 \% & HDF5 shuffle ('SZIP', 'nn', 24) all-row-chunk & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4hc') all-row-chunk & 68.8 \% & HDF5 no-shuffle ('SZIP', 'ec', 4) all-row-chunk & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4hc') all-row-chunk & 68.8 \% & HDF5 shuffle ('SZIP', 'ec', 32) all-row-chunk & 200.1 \% \\
Zarr Blosc(cname='blosclz', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 69.7 \% & HDF5 shuffle ('SZIP', 'ec', 4) all-row-chunk & 200.1 \% \\
HDF5 no-shuffle bitshuffle-lz4 all-row-chunk & 69.9 \% & HDF5 no-shuffle ('SZIP', 'nn', 2) all-row-chunk & 200.1 \% \\
HDF5 no-shuffle ('SZIP', 'nn', 24) all-column-chunk & 70.8 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'blosclz') all-row-chunk & 200.1 \% \\
HDF5 no-shuffle ('SZIP', 'nn', 24) individual-dsets & 70.9 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'blosclz') all-row-chunk & 200.1 \% \\
Zarr Blosc(cname='snappy', shuffle=BITSHUFFLE, blocksize=0) & 72.6 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'blosclz') all-column-chunk & 200.1 \% \\
Zarr Blosc(cname='lz4', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 73.2 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'blosclz') all-column-chunk & 200.1 \% \\
HDF5 shuffle bitshuffle-lz4 all-row-chunk & 74.8 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'blosclz') all-row-chunk & 200.1 \% \\
HDF5 no-shuffle gzip all-row-chunk & 76.1 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'blosclz') all-row-chunk & 200.1 \% \\
HDF5 no-shuffle ('SZIP', 'nn', 32) all-column-chunk & 76.8 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'blosclz') all-row-chunk & 200.1 \% \\
HDF5 no-shuffle ('SZIP', 'nn', 32) individual-dsets & 76.8 \% & HDF5 shuffle ('SZIP', 'ec', 2) all-row-chunk & 200.1 \% \\
Zarr Blosc(cname='lz4', shuffle=NOSHUFFLE, blocksize=0) & 79.5 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'blosclz') all-column-chunk & 200.1 \% \\
Zarr Blosc(cname='snappy', shuffle=NOSHUFFLE, blocksize=0) & 80.2 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'blosclz') all-row-chunk & 200.1 \% \\
Zarr Blosc(cname='blosclz', shuffle=NOSHUFFLE, blocksize=0) & 82.3 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'blosclz') all-column-chunk & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4') all-column-chunk & 85.4 \% & HDF5 no-shuffle ('SZIP', 'ec', 2) all-row-chunk & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4') all-column-chunk & 85.4 \% & HDF5 shuffle ('SZIP', 'ec', 32) all-column-chunk & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4') all-column-chunk & 85.4 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'blosclz') all-column-chunk & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4') all-column-chunk & 85.4 \% & HDF5 shuffle ('SZIP', 'nn', 32) all-row-chunk & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4') all-column-chunk & 85.4 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'blosclz') all-row-chunk & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4') all-column-chunk & 85.4 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'blosclz') all-row-chunk & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4') all-column-chunk & 85.4 \% & HDF5 shuffle ('SZIP', 'nn', 2) all-row-chunk & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4') all-column-chunk & 85.4 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'blosclz') all-row-chunk & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4') all-column-chunk & 85.4 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'blosclz') all-column-chunk & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4') individual-dsets & 86.0 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'blosclz') all-column-chunk & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4') individual-dsets & 86.0 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'blosclz') all-column-chunk & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4') individual-dsets & 86.0 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'blosclz') all-column-chunk & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4') individual-dsets & 86.0 \% & HDF5 shuffle ('SZIP', 'ec', 32) individual-dsets & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4') individual-dsets & 86.0 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'blosclz') individual-dsets & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4') individual-dsets & 86.0 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'blosclz') individual-dsets & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4') individual-dsets & 86.0 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'blosclz') individual-dsets & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4') individual-dsets & 86.0 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'blosclz') individual-dsets & 200.1 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4') individual-dsets & 86.0 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'blosclz') individual-dsets & 200.1 \% \\
HDF5 shuffle ('SZIP', 'nn', 2) all-column-chunk & 88.4 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'blosclz') individual-dsets & 200.1 \% \\
HDF5 shuffle ('SZIP', 'nn', 2) individual-dsets & 88.4 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'blosclz') individual-dsets & 200.1 \% \\
HDF5 shuffle ('SZIP', 'nn', 4) all-column-chunk & 89.6 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'blosclz') individual-dsets & 200.1 \% \\
HDF5 shuffle ('SZIP', 'nn', 4) individual-dsets & 89.6 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'blosclz') individual-dsets & 200.1 \% \\
Zarr Blosc(cname='snappy', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 94.9 \%  \\
Zarr Blosc(cname='snappy', shuffle=SHUFFLE, blocksize=0) & 96.1 \%  \\
RAW-UNCOMPRESSED & 100.0 \%  \\
Zarr None (Delta(dtype='<i2'),) & 100.0 \%  \\
Zarr None & 100.0 \%  \\
HDF5 shuffle ('SZIP', 'nn', 8) all-column-chunk & 101.3 \%  \\
HDF5 shuffle ('SZIP', 'nn', 8) individual-dsets & 101.4 \%  \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4') all-row-chunk & 115.0 \%  \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4') all-row-chunk & 115.0 \%  \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4') all-row-chunk & 115.0 \%  \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4') all-row-chunk & 115.0 \%  \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4') all-row-chunk & 115.0 \%  \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4') all-row-chunk & 115.0 \%  \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4') all-row-chunk & 115.0 \%  \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4') all-row-chunk & 115.0 \%  \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4') all-row-chunk & 115.0 \%  \\
HDF5 shuffle ('SZIP', 'nn', 16) all-column-chunk & 126.6 \%  \\
HDF5 shuffle ('SZIP', 'nn', 16) individual-dsets & 126.7 \%  \\
HDF5 no-shuffle lzf all-column-chunk & 128.4 \%  \\
HDF5 no-shuffle lzf individual-dsets & 128.4 \%  \\
HDF5 no-shuffle lzf all-row-chunk & 139.5 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 8) all-column-chunk & 142.8 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 8) individual-dsets & 142.8 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 16) all-column-chunk & 144.6 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 16) individual-dsets & 144.7 \%  \\
HDF5 shuffle ('SZIP', 'nn', 24) all-column-chunk & 146.5 \%  \\
HDF5 shuffle ('SZIP', 'nn', 24) individual-dsets & 146.5 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 4) all-column-chunk & 146.8 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 4) individual-dsets & 146.9 \%  \\
HDF5 shuffle ('SZIP', 'nn', 32) all-column-chunk & 148.2 \%  \\
HDF5 shuffle ('SZIP', 'nn', 32) individual-dsets & 148.2 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 24) all-column-chunk & 148.5 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 24) individual-dsets & 148.6 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 32) all-column-chunk & 153.0 \%  \\
\end{longtable}
\tiny \begin{longtable}{lc|lc}
\caption{UK-DALE: Data representation benchmark \numberOfDataRepresentations{} formats and data transformations. Raw input data size was \SI{6259.4}{\gibi\byte} from 19486 files.} \\
\textbf{Name} & \textbf{Compression Ratio} & \textbf{Name} & \textbf{Compression Ratio} \\ \hline \endhead
HDF5 no-shuffle MAFISC-LZMA all-column-chunk & 59.5 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'snappy') individual-dsets & 76.4 \% \\
ALAC PCM-24 & 60.2 \% & HDF5 no-shuffle ('SZIP', 'nn', 16) all-column-chunk & 76.5 \% \\
FLAC PCM-24 & 61.0 \% & HDF5 no-shuffle ('SZIP', 'nn', 16) individual-dsets & 76.5 \% \\
HDF5 shuffle zstd all-column-chunk & 63.3 \% & HDF5 no-shuffle ('SZIP', 'nn', 24) all-column-chunk & 77.6 \% \\
HDF5 shuffle zstd individual-dsets & 63.4 \% & HDF5 no-shuffle ('SZIP', 'nn', 24) individual-dsets & 77.6 \% \\
HDF5 no-shuffle MAFISC-LZMA individual-dsets & 63.6 \% & ZLIB LEB128S-delta-column & 77.7 \% \\
WavPack PCM-24 & 64.3 \% & LZMA raw-row DELTA distance-3 & 77.8 \% \\
Zarr Blosc-zstd SHUFFLE Delta & 65.3 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zstd') all-row-chunk & 77.9 \% \\
LZMA-alone LEB128S-delta-row & 65.8 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zstd') all-row-chunk & 77.9 \% \\
LZMA-xz LEB128S-delta-row & 65.8 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zstd') all-row-chunk & 77.9 \% \\
bzip2 LEB128S-delta-row & 66.9 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zstd') all-row-chunk & 77.9 \% \\
Zarr Blosc(cname='zlib', SHUFFLE Delta & 67.0 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zstd') all-row-chunk & 77.9 \% \\
Zarr Blosc-zstd SHUFFLE & 67.0 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zstd') all-row-chunk & 77.9 \% \\
Zarr LZMA Delta & 67.5 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zstd') all-row-chunk & 77.9 \% \\
HDF5 shuffle zstd all-row-chunk & 67.5 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zstd') all-row-chunk & 77.9 \% \\
HDF5 shuffle gzip all-column-chunk & 67.7 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zstd') all-row-chunk & 77.9 \% \\
HDF5 shuffle gzip individual-dsets & 67.7 \% & HDF5 shuffle lzf all-row-chunk & 78.2 \% \\
Zarr Blosc(cname='zlib', SHUFFLE & 68.3 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zlib') all-row-chunk & 78.3 \% \\
Zarr Blosc(cname='lz4hc', SHUFFLE & 69.0 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zlib') all-row-chunk & 78.3 \% \\
Zarr BZ2 Delta & 69.0 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zlib') all-row-chunk & 78.3 \% \\
HDF5 shuffle gzip all-row-chunk & 69.1 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zlib') all-row-chunk & 78.3 \% \\
HDF5 shuffle MAFISC-LZMA individual-dsets & 69.2 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zlib') all-row-chunk & 78.3 \% \\
LZMA raw-column DELTA distance-3 & 69.5 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zlib') all-row-chunk & 78.3 \% \\
Zarr Blosc(cname='lz4hc', SHUFFLE Delta & 70.6 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zlib') all-row-chunk & 78.3 \% \\
Zarr LZMA & 70.6 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zlib') all-row-chunk & 78.3 \% \\
LZMA-alone LEB128S-row & 71.2 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zlib') all-row-chunk & 78.3 \% \\
LZMA-xz LEB128S-row & 71.2 \% & HDF5 no-shuffle ('SZIP', 'nn', 4) all-column-chunk & 78.4 \% \\
zstd-22 LEB128S-delta-row & 71.4 \% & HDF5 no-shuffle ('SZIP', 'nn', 4) individual-dsets & 78.4 \% \\
LZMA-alone LEB128S-delta-column & 71.5 \% & LZMA-alone LEB128S-column & 78.4 \% \\
LZMA-xz LEB128S-delta-column & 71.6 \% & LZMA-xz LEB128S-column & 78.4 \% \\
LZMA LEB128S-delta-row DELTA distance-3 & 71.8 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'snappy') all-row-chunk & 78.4 \% \\
bzip2 LEB128S-delta-column & 72.3 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'snappy') all-row-chunk & 78.4 \% \\
HDF5 shuffle MAFISC-LZMA all-row-chunk & 72.3 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'snappy') all-row-chunk & 78.4 \% \\
LZMA-alone raw-column & 72.6 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'snappy') all-row-chunk & 78.4 \% \\
LZMA-xz raw-column & 72.6 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'snappy') all-row-chunk & 78.4 \% \\
Zarr Blosc(cname='lz4', SHUFFLE & 74.3 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'snappy') all-row-chunk & 78.4 \% \\
LZMA-alone raw-row & 74.5 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'snappy') all-row-chunk & 78.4 \% \\
LZMA-xz raw-row & 74.5 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'snappy') all-row-chunk & 78.4 \% \\
Zarr Blosc(cname='snappy', SHUFFLE & 74.5 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'snappy') all-row-chunk & 78.4 \% \\
LZMA LEB128S-delta-row DELTA distance-1 & 75.1 \% & HDF5 shuffle bitshuffle-lz4 all-column-chunk & 78.8 \% \\
zstd-22 LEB128S-delta-column & 75.3 \% & HDF5 shuffle bitshuffle-lz4 individual-dsets & 78.8 \% \\
HDF5 no-shuffle MAFISC-LZMA all-row-chunk & 75.7 \% & Zarr Blosc(cname='blosclz', SHUFFLE & 78.9 \% \\
HDF5 no-shuffle ('SZIP', 'nn', 8) all-column-chunk & 76.0 \% & HDF5 no-shuffle ('SZIP', 'nn', 32) all-column-chunk & 78.9 \% \\
HDF5 no-shuffle ('SZIP', 'nn', 8) individual-dsets & 76.0 \% & HDF5 no-shuffle ('SZIP', 'nn', 32) individual-dsets & 78.9 \% \\
HDF5 shuffle lzf all-column-chunk & 76.0 \% & Zarr Blosc(cname='snappy', SHUFFLE Delta & 80.1 \% \\
HDF5 shuffle lzf individual-dsets & 76.0 \% & HDF5 shuffle bitshuffle-lz4 all-row-chunk & 80.4 \% \\
ZLIB LEB128S-delta-row & 76.2 \% & LZMA LEB128S-delta-row DELTA distance-2 & 80.7 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zstd') individual-dsets & 76.2 \% & Zarr Blosc-zstd BITSHUFFLE Delta & 80.9 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zstd') individual-dsets & 76.2 \% & Zarr Blosc-zstd NOSHUFFLE Delta & 81.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zstd') individual-dsets & 76.2 \% & LZMA LEB128S-delta-row DELTA distance-4 & 81.3 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zstd') individual-dsets & 76.2 \% & LZMA LEB128S-delta-column DELTA distance-3 & 81.3 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zstd') individual-dsets & 76.2 \% & LZMA LEB128S-delta-column DELTA distance-1 & 81.7 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zstd') individual-dsets & 76.2 \% & HDF5 no-shuffle bitshuffle-lz4 all-column-chunk & 81.8 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zstd') individual-dsets & 76.2 \% & HDF5 no-shuffle bitshuffle-lz4 individual-dsets & 81.8 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zstd') individual-dsets & 76.2 \% & LZMA LEB128S-delta-column DELTA distance-2 & 82.2 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zstd') individual-dsets & 76.2 \% & LZMA LEB128S-delta-column DELTA distance-4 & 82.2 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zstd') all-column-chunk & 76.2 \% & Zarr Blosc(cname='lz4', SHUFFLE Delta & 83.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zstd') all-column-chunk & 76.2 \% & HDF5 shuffle ('SZIP', 'nn', 8) all-row-chunk & 83.5 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zstd') all-column-chunk & 76.2 \% & HDF5 no-shuffle ('SZIP', 'nn', 2) all-column-chunk & 84.7 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zstd') all-column-chunk & 76.2 \% & HDF5 no-shuffle ('SZIP', 'nn', 2) individual-dsets & 84.7 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zstd') all-column-chunk & 76.2 \% & HDF5 shuffle ('SZIP', 'nn', 4) all-row-chunk & 85.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zstd') all-column-chunk & 76.2 \% & HDF5 shuffle ('SZIP', 'nn', 16) all-row-chunk & 85.2 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zstd') all-column-chunk & 76.2 \% & zstd-22 raw-column & 85.3 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zstd') all-column-chunk & 76.2 \% & Zarr Blosc(cname='blosclz', SHUFFLE Delta & 85.7 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zstd') all-column-chunk & 76.2 \% & bzip2 raw-column & 86.9 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zlib') individual-dsets & 76.4 \% & HDF5 shuffle ('SZIP', 'nn', 24) all-row-chunk & 87.5 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zlib') individual-dsets & 76.4 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4hc') all-column-chunk & 87.6 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zlib') individual-dsets & 76.4 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4hc') all-column-chunk & 87.6 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zlib') individual-dsets & 76.4 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4hc') all-column-chunk & 87.6 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zlib') individual-dsets & 76.4 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4hc') all-column-chunk & 87.6 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zlib') individual-dsets & 76.4 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4hc') all-column-chunk & 87.6 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zlib') individual-dsets & 76.4 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4hc') all-column-chunk & 87.6 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zlib') individual-dsets & 76.4 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4hc') all-column-chunk & 87.6 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zlib') individual-dsets & 76.4 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4hc') all-column-chunk & 87.6 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zlib') all-column-chunk & 76.4 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4hc') all-column-chunk & 87.6 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zlib') all-column-chunk & 76.4 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4hc') individual-dsets & 87.6 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zlib') all-column-chunk & 76.4 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4hc') individual-dsets & 87.6 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zlib') all-column-chunk & 76.4 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4hc') individual-dsets & 87.6 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zlib') all-column-chunk & 76.4 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4hc') individual-dsets & 87.6 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zlib') all-column-chunk & 76.4 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4hc') individual-dsets & 87.6 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zlib') all-column-chunk & 76.4 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4hc') individual-dsets & 87.6 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zlib') all-column-chunk & 76.4 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4hc') individual-dsets & 87.6 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zlib') all-column-chunk & 76.4 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4hc') individual-dsets & 87.6 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'snappy') all-column-chunk & 76.4 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4hc') individual-dsets & 87.6 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'snappy') all-column-chunk & 76.4 \% & Zarr Blosc(cname='zlib', BITSHUFFLE Delta & 88.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'snappy') all-column-chunk & 76.4 \% & Zarr Zlib(level=9) Delta & 88.1 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'snappy') all-column-chunk & 76.4 \% & Zarr Blosc(cname='zlib', NOSHUFFLE Delta & 88.1 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'snappy') all-column-chunk & 76.4 \% & HDF5 no-shuffle bitshuffle-lz4 all-row-chunk & 88.3 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'snappy') all-column-chunk & 76.4 \% & zstd-22 LEB128S-row & 88.6 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'snappy') all-column-chunk & 76.4 \% & LZMA LEB128S-row DELTA distance-4 & 89.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'snappy') all-column-chunk & 76.4 \% & HDF5 no-shuffle zstd all-column-chunk & 89.7 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'snappy') all-column-chunk & 76.4 \% & HDF5 no-shuffle zstd individual-dsets & 89.7 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'snappy') individual-dsets & 76.4 \% & HDF5 shuffle ('SZIP', 'nn', 32) all-row-chunk & 89.9 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'snappy') individual-dsets & 76.4 \% & zstd-22 raw-row & 90.8 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'snappy') individual-dsets & 76.4 \% & LZMA raw-column DELTA distance-1 & 91.5 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'snappy') individual-dsets & 76.4 \% & bzip2 LEB128S-row & 92.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'snappy') individual-dsets & 76.4 \% & HDF5 shuffle ('SZIP', 'nn', 8) all-column-chunk & 92.5 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'snappy') individual-dsets & 76.4 \% & HDF5 shuffle ('SZIP', 'nn', 8) individual-dsets & 92.5 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'snappy') individual-dsets & 76.4 \% & HDF5 shuffle ('SZIP', 'nn', 4) all-column-chunk & 92.6 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'snappy') individual-dsets & 76.4 \% & HDF5 shuffle ('SZIP', 'nn', 4) individual-dsets & 92.6 \% \\
ZLIB raw-column & 92.9 \% & HDF5 no-shuffle ('SZIP', 'ec', 16) all-row-chunk & 122.3 \% \\
HDF5 no-shuffle zstd all-row-chunk & 93.4 \% & HDF5 shuffle ('SZIP', 'ec', 16) all-column-chunk & 122.8 \% \\
zstd-22 LEB128S-column & 94.7 \% & HDF5 shuffle ('SZIP', 'ec', 16) individual-dsets & 122.8 \% \\
Zarr BZ2 & 95.2 \% & HDF5 shuffle ('SZIP', 'ec', 4) all-column-chunk & 123.6 \% \\
ZLIB raw-row & 95.5 \% & HDF5 shuffle ('SZIP', 'ec', 4) individual-dsets & 123.6 \% \\
bzip2 raw-row & 96.8 \% & HDF5 no-shuffle ('SZIP', 'ec', 8) all-row-chunk & 124.6 \% \\
LZMA LEB128S-row DELTA distance-1 & 97.0 \% & HDF5 shuffle ('SZIP', 'ec', 24) all-column-chunk & 126.0 \% \\
HDF5 shuffle ('SZIP', 'nn', 16) all-column-chunk & 97.2 \% & HDF5 shuffle ('SZIP', 'ec', 24) individual-dsets & 126.0 \% \\
HDF5 shuffle ('SZIP', 'nn', 16) individual-dsets & 97.2 \% & Zarr Blosc(cname='lz4hc', BITSHUFFLE & 128.8 \% \\
LZMA LEB128S-row DELTA distance-2 & 97.6 \% & Zarr Blosc(cname='lz4hc', NOSHUFFLE & 128.9 \% \\
HDF5 shuffle ('SZIP', 'nn', 2) all-column-chunk & 97.9 \% & HDF5 no-shuffle ('SZIP', 'ec', 2) individual-dsets & 129.1 \% \\
HDF5 shuffle ('SZIP', 'nn', 2) individual-dsets & 97.9 \% & Zarr Blosc(cname='snappy', BITSHUFFLE Delta & 129.1 \% \\
LZMA LEB128S-row DELTA distance-3 & 98.3 \% & Zarr Blosc(cname='snappy', NOSHUFFLE Delta & 129.2 \% \\
bzip2 LEB128S-column & 98.5 \% & HDF5 shuffle ('SZIP', 'ec', 32) individual-dsets & 129.5 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4hc') all-row-chunk & 98.9 \% & HDF5 shuffle ('SZIP', 'ec', 32) all-column-chunk & 129.5 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4hc') all-row-chunk & 98.9 \% & HDF5 no-shuffle ('SZIP', 'ec', 4) all-row-chunk & 129.7 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4hc') all-row-chunk & 98.9 \% & HDF5 shuffle ('SZIP', 'ec', 2) individual-dsets & 130.2 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4hc') all-row-chunk & 98.9 \% & HDF5 no-shuffle ('SZIP', 'ec', 2) all-column-chunk & 130.4 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4hc') all-row-chunk & 98.9 \% & Zarr Blosc(cname='lz4', BITSHUFFLE Delta & 130.5 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4hc') all-row-chunk & 98.9 \% & Zarr Blosc(cname='lz4', NOSHUFFLE Delta & 130.6 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4hc') all-row-chunk & 98.9 \% & Zarr Blosc(cname='blosclz', BITSHUFFLE Delta & 131.2 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4hc') all-row-chunk & 98.9 \% & Zarr Blosc(cname='blosclz', NOSHUFFLE Delta & 131.4 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4hc') all-row-chunk & 98.9 \% & HDF5 no-shuffle lzf individual-dsets & 131.6 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4') all-column-chunk & 99.6 \% & HDF5 shuffle MAFISC-LZMA all-column-chunk & 131.7 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4') all-column-chunk & 99.6 \% & HDF5 shuffle ('SZIP', 'nn', 2) all-row-chunk & 132.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4') all-column-chunk & 99.6 \% & HDF5 shuffle ('SZIP', 'ec', 2) all-column-chunk & 132.1 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4') all-column-chunk & 99.6 \% & HDF5 no-shuffle lzf all-column-chunk & 132.5 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4') all-column-chunk & 99.6 \% & HDF5 no-shuffle lzf all-row-chunk & 132.6 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4') all-column-chunk & 99.6 \% & Zarr Blosc(cname='lz4', BITSHUFFLE & 133.2 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4') all-column-chunk & 99.6 \% & Zarr Blosc(cname='snappy', BITSHUFFLE & 133.3 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4') all-column-chunk & 99.6 \% & Zarr Blosc(cname='lz4', NOSHUFFLE & 133.4 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4') all-column-chunk & 99.6 \% & Zarr Blosc(cname='blosclz', BITSHUFFLE & 133.4 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4') individual-dsets & 99.6 \% & Zarr Blosc(cname='snappy', NOSHUFFLE & 133.5 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4') individual-dsets & 99.6 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'blosclz') all-column-chunk & 133.5 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4') individual-dsets & 99.6 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'blosclz') all-row-chunk & 133.5 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4') individual-dsets & 99.6 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'blosclz') all-row-chunk & 133.5 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4') individual-dsets & 99.6 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'blosclz') all-column-chunk & 133.5 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4') individual-dsets & 99.6 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'blosclz') all-column-chunk & 133.5 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4') individual-dsets & 99.6 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'blosclz') all-row-chunk & 133.5 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4') individual-dsets & 99.6 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'blosclz') all-row-chunk & 133.5 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4') individual-dsets & 99.6 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'blosclz') all-row-chunk & 133.5 \% \\
LZMA raw-column DELTA distance-2 & 99.7 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'blosclz') all-row-chunk & 133.5 \% \\
RAW-UNCOMPRESSED & 100.0 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'blosclz') all-column-chunk & 133.5 \% \\
LZMA raw-column DELTA distance-4 & 100.0 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'blosclz') all-column-chunk & 133.5 \% \\
LZMA raw-row DELTA distance-1 & 100.0 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'blosclz') all-row-chunk & 133.5 \% \\
LZMA raw-row DELTA distance-4 & 100.0 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'blosclz') all-column-chunk & 133.5 \% \\
LZMA raw-row DELTA distance-2 & 100.0 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'blosclz') all-column-chunk & 133.5 \% \\
ZLIB LEB128S-row & 100.5 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'blosclz') all-column-chunk & 133.5 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4') all-row-chunk & 101.1 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'blosclz') all-row-chunk & 133.5 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4') all-row-chunk & 101.1 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'blosclz') all-row-chunk & 133.5 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4') all-row-chunk & 101.1 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'blosclz') all-column-chunk & 133.5 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4') all-row-chunk & 101.1 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'blosclz') individual-dsets & 133.5 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4') all-row-chunk & 101.1 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'blosclz') individual-dsets & 133.5 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4') all-row-chunk & 101.1 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'blosclz') individual-dsets & 133.5 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4') all-row-chunk & 101.1 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'blosclz') individual-dsets & 133.5 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4') all-row-chunk & 101.1 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'blosclz') individual-dsets & 133.5 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4') all-row-chunk & 101.1 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'blosclz') individual-dsets & 133.5 \% \\
Zarr Blosc-zstd BITSHUFFLE & 101.2 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'blosclz') individual-dsets & 133.5 \% \\
Zarr Blosc-zstd NOSHUFFLE & 101.3 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'blosclz') individual-dsets & 133.5 \% \\
HDF5 shuffle ('SZIP', 'nn', 24) all-column-chunk & 101.6 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'blosclz') individual-dsets & 133.5 \% \\
HDF5 shuffle ('SZIP', 'nn', 24) individual-dsets & 101.6 \% & Zarr None & 133.5 \% \\
ZLIB LEB128S-column & 102.6 \% & Zarr None Delta & 133.5 \% \\
LZMA LEB128S-column DELTA distance-3 & 106.0 \% & HDF5 no-shuffle ('SZIP', 'nn', 2) all-row-chunk & 133.5 \% \\
HDF5 no-shuffle gzip all-column-chunk & 106.0 \% & HDF5 shuffle ('SZIP', 'ec', 2) all-row-chunk & 133.5 \% \\
HDF5 no-shuffle gzip individual-dsets & 106.0 \% & HDF5 no-shuffle ('SZIP', 'ec', 2) all-row-chunk & 133.5 \% \\
HDF5 shuffle ('SZIP', 'nn', 32) all-column-chunk & 106.0 \% & Zarr Blosc(cname='blosclz', NOSHUFFLE & 133.5 \% \\
HDF5 shuffle ('SZIP', 'nn', 32) individual-dsets & 106.0 \%  \\
Zarr Blosc(cname='zlib', BITSHUFFLE & 106.0 \%  \\
Zarr Zlib(level=9) & 106.1 \%  \\
Zarr Blosc(cname='zlib', NOSHUFFLE & 106.1 \%  \\
LZMA LEB128S-column DELTA distance-4 & 107.3 \%  \\
LZMA LEB128S-column DELTA distance-1 & 108.2 \%  \\
HDF5 no-shuffle gzip all-row-chunk & 109.5 \%  \\
Zarr Blosc(cname='lz4hc', BITSHUFFLE Delta & 109.9 \%  \\
Zarr Blosc(cname='lz4hc', NOSHUFFLE Delta & 110.1 \%  \\
HDF5 no-shuffle ('SZIP', 'nn', 16) all-row-chunk & 110.2 \%  \\
HDF5 no-shuffle ('SZIP', 'nn', 24) all-row-chunk & 110.3 \%  \\
HDF5 no-shuffle ('SZIP', 'nn', 32) all-row-chunk & 110.8 \%  \\
HDF5 no-shuffle ('SZIP', 'nn', 8) all-row-chunk & 111.5 \%  \\
LZMA LEB128S-column DELTA distance-2 & 113.7 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 16) all-column-chunk & 115.5 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 16) individual-dsets & 115.5 \%  \\
HDF5 no-shuffle ('SZIP', 'nn', 4) all-row-chunk & 115.7 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 24) all-column-chunk & 116.0 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 24) individual-dsets & 116.0 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 8) all-column-chunk & 116.7 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 8) individual-dsets & 116.7 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 32) all-column-chunk & 116.8 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 32) individual-dsets & 116.8 \%  \\
HDF5 shuffle ('SZIP', 'ec', 16) all-row-chunk & 118.2 \%  \\
HDF5 shuffle ('SZIP', 'ec', 8) all-row-chunk & 118.3 \%  \\
HDF5 shuffle ('SZIP', 'ec', 24) all-row-chunk & 119.6 \%  \\
HDF5 shuffle ('SZIP', 'ec', 8) all-column-chunk & 120.9 \%  \\
HDF5 shuffle ('SZIP', 'ec', 8) individual-dsets & 120.9 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 4) all-column-chunk & 121.0 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 4) individual-dsets & 121.0 \%  \\
HDF5 shuffle ('SZIP', 'ec', 32) all-row-chunk & 121.4 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 32) all-row-chunk & 121.9 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 24) all-row-chunk & 121.9 \%  \\
HDF5 shuffle ('SZIP', 'ec', 4) all-row-chunk & 122.0 \%  \\
\end{longtable}
\tiny \begin{longtable}{lc|lc}
\caption{BLOND-50: Data representation benchmark \numberOfDataRepresentations{} formats and data transformations. Raw input data size was \SI{10246.7}{\gibi\byte} from 61124 files.} \\
\textbf{Name} & \textbf{Compression Ratio} & \textbf{Name} & \textbf{Compression Ratio} \\ \hline \endhead
ALAC PCM-16 & 48.7 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zstd') all-column-chunk & 87.4 \% \\
HDF5 no-shuffle MAFISC-LZMA all-column-chunk & 52.9 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zstd') individual-dsets & 87.5 \% \\
FLAC PCM-16 & 54.4 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zstd') individual-dsets & 87.5 \% \\
Zarr BZ2 (Delta(dtype='<i2'),) & 54.8 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zstd') individual-dsets & 87.5 \% \\
LZMA-alone LEB128S-delta-row & 55.9 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zstd') individual-dsets & 87.5 \% \\
LZMA-xz LEB128S-delta-row & 55.9 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zstd') individual-dsets & 87.5 \% \\
bzip2 LEB128S-delta-row & 56.1 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zstd') individual-dsets & 87.5 \% \\
WavPack PCM-16 & 56.8 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zstd') individual-dsets & 87.5 \% \\
Zarr Blosc-zstd shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 57.7 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zstd') individual-dsets & 87.5 \% \\
Zarr LZMA (Delta(dtype='<i2'),) & 58.3 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zstd') individual-dsets & 87.5 \% \\
LZMA raw-column DELTA distance-2 & 58.3 \% & zstd-22 raw-row & 88.5 \% \\
Zarr Blosc(cname='zlib', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 58.7 \% & Zarr Blosc(cname='lz4hc', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 89.1 \% \\
HDF5 shuffle zstd individual-dsets & 58.7 \% & ZLIB raw-column & 89.3 \% \\
Zarr Blosc(cname='zlib', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 58.9 \% & Zarr Zlib(level=9) & 89.3 \% \\
Zarr Blosc-zstd shuffle=SHUFFLE, blocksize=0) & 59.0 \% & Zarr Blosc(cname='zlib', shuffle=NOSHUFFLE, blocksize=0) & 89.5 \% \\
HDF5 shuffle zstd all-column-chunk & 59.3 \% & zstd-22 LEB128S-column & 92.1 \% \\
LZMA-alone raw-column & 60.0 \% & bzip2 raw-row & 92.8 \% \\
LZMA-xz raw-column & 60.0 \% & ZLIB raw-row & 93.9 \% \\
LZMA raw-column DELTA distance-4 & 60.2 \% & Zarr Blosc(cname='lz4', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 94.5 \% \\
LZMA-alone LEB128S-row & 60.6 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zlib') all-column-chunk & 94.7 \% \\
LZMA-xz LEB128S-row & 60.6 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zlib') all-column-chunk & 94.7 \% \\
zstd-22 LEB128S-delta-row & 60.9 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zlib') all-column-chunk & 94.7 \% \\
Zarr Blosc(cname='lz4hc', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 61.0 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zlib') all-column-chunk & 94.7 \% \\
Zarr Blosc(cname='zlib', shuffle=SHUFFLE, blocksize=0) & 61.3 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zlib') all-column-chunk & 94.7 \% \\
LZMA-alone LEB128S-delta-column & 61.4 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zlib') all-column-chunk & 94.7 \% \\
LZMA-xz LEB128S-delta-column & 61.4 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zlib') all-column-chunk & 94.7 \% \\
Zarr Blosc(cname='lz4hc', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 61.9 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zlib') all-column-chunk & 94.7 \% \\
Zarr Blosc(cname='lz4', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 62.5 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zlib') all-column-chunk & 94.7 \% \\
HDF5 shuffle zstd all-row-chunk & 63.1 \% & LZMA raw-row DELTA distance-1 & 94.8 \% \\
LZMA raw-column DELTA distance-1 & 63.1 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zlib') individual-dsets & 94.9 \% \\
Zarr LZMA & 63.6 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zlib') individual-dsets & 94.9 \% \\
HDF5 shuffle gzip all-column-chunk & 63.9 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zlib') individual-dsets & 94.9 \% \\
HDF5 shuffle gzip individual-dsets & 64.0 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zlib') individual-dsets & 94.9 \% \\
Zarr Blosc(cname='lz4hc', shuffle=SHUFFLE, blocksize=0) & 64.9 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zlib') individual-dsets & 94.9 \% \\
Zarr Blosc(cname='zlib', shuffle=BITSHUFFLE, blocksize=0) & 65.3 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zlib') individual-dsets & 94.9 \% \\
Zarr Blosc-zstd shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 65.4 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zlib') individual-dsets & 94.9 \% \\
Zarr Blosc-zstd shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 65.4 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zlib') individual-dsets & 94.9 \% \\
LZMA LEB128S-delta-row DELTA distance-2 & 65.5 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zlib') individual-dsets & 94.9 \% \\
LZMA LEB128S-delta-row DELTA distance-1 & 65.8 \% & bzip2 LEB128S-column & 94.9 \% \\
bzip2 LEB128S-delta-column & 66.4 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'snappy') all-column-chunk & 95.9 \% \\
Zarr Blosc(cname='blosclz', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 66.4 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'snappy') all-column-chunk & 95.9 \% \\
HDF5 no-shuffle zstd all-column-chunk & 66.4 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'snappy') all-column-chunk & 95.9 \% \\
HDF5 no-shuffle zstd individual-dsets & 66.5 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'snappy') all-column-chunk & 95.9 \% \\
HDF5 no-shuffle MAFISC-LZMA individual-dsets & 66.6 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'snappy') all-column-chunk & 95.9 \% \\
bzip2 raw-column & 67.2 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'snappy') all-column-chunk & 95.9 \% \\
zstd-22 LEB128S-delta-column & 67.3 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'snappy') all-column-chunk & 95.9 \% \\
LZMA LEB128S-delta-row DELTA distance-4 & 67.5 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'snappy') all-column-chunk & 95.9 \% \\
bzip2 LEB128S-row & 67.6 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'snappy') all-column-chunk & 95.9 \% \\
Zarr BZ2 & 67.8 \% & HDF5 no-shuffle ('SZIP', 'nn', 4) all-column-chunk & 96.0 \% \\
ZLIB LEB128S-delta-row & 68.3 \% & HDF5 no-shuffle ('SZIP', 'nn', 4) individual-dsets & 96.0 \% \\
Zarr Blosc(cname='blosclz', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 68.8 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'snappy') individual-dsets & 96.1 \% \\
Zarr Blosc(cname='lz4hc', shuffle=BITSHUFFLE, blocksize=0) & 69.3 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'snappy') individual-dsets & 96.1 \% \\
Zarr Blosc(cname='lz4', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 69.3 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'snappy') individual-dsets & 96.1 \% \\
Zarr Zlib(level=9) (Delta(dtype='<i2'),) & 70.2 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'snappy') individual-dsets & 96.1 \% \\
Zarr Blosc(cname='zlib', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 70.9 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'snappy') individual-dsets & 96.1 \% \\
zstd-22 raw-column & 71.3 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'snappy') individual-dsets & 96.1 \% \\
HDF5 no-shuffle zstd all-row-chunk & 71.6 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'snappy') individual-dsets & 96.1 \% \\
zstd-22 LEB128S-row & 72.4 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'snappy') individual-dsets & 96.1 \% \\
Zarr Blosc(cname='lz4', shuffle=BITSHUFFLE, blocksize=0) & 73.1 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'snappy') individual-dsets & 96.1 \% \\
ZLIB LEB128S-delta-column & 73.3 \% & ZLIB LEB128S-row & 96.1 \% \\
Zarr Blosc(cname='lz4', shuffle=SHUFFLE, blocksize=0) & 73.6 \% & HDF5 no-shuffle ('SZIP', 'nn', 8) all-column-chunk & 96.8 \% \\
HDF5 no-shuffle MAFISC-LZMA all-row-chunk & 73.9 \% & HDF5 no-shuffle ('SZIP', 'nn', 8) individual-dsets & 96.8 \% \\
LZMA-alone raw-row & 74.0 \% & HDF5 no-shuffle bitshuffle-lz4 all-row-chunk & 97.3 \% \\
LZMA-xz raw-row & 74.0 \% & Zarr Blosc(cname='snappy', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 98.0 \% \\
HDF5 shuffle MAFISC-LZMA individual-dsets & 74.7 \% & Zarr Blosc(cname='blosclz', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 98.2 \% \\
LZMA LEB128S-delta-row DELTA distance-3 & 74.9 \% & Zarr Blosc(cname='lz4hc', shuffle=NOSHUFFLE, blocksize=0) & 98.9 \% \\
HDF5 shuffle gzip all-row-chunk & 75.0 \% & Zarr Blosc(cname='snappy', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 99.4 \% \\
LZMA LEB128S-row DELTA distance-3 & 75.1 \% & Zarr Blosc(cname='lz4', shuffle=NOSHUFFLE, blocksize=0) & 100.0 \% \\
LZMA LEB128S-row DELTA distance-2 & 75.4 \% & Zarr None (Delta(dtype='<i2'),) & 100.0 \% \\
Zarr Blosc(cname='blosclz', shuffle=BITSHUFFLE, blocksize=0) & 76.0 \% & Zarr None & 100.0 \% \\
LZMA LEB128S-row DELTA distance-1 & 76.5 \% & RAW-UNCOMPRESSED & 100.0 \% \\
Zarr Blosc(cname='blosclz', shuffle=SHUFFLE, blocksize=0) & 76.7 \% & Zarr Blosc(cname='snappy', shuffle=BITSHUFFLE, blocksize=0) & 100.0 \% \\
LZMA-alone LEB128S-column & 77.1 \% & Zarr Blosc(cname='snappy', shuffle=NOSHUFFLE, blocksize=0) & 100.0 \% \\
LZMA-xz LEB128S-column & 77.1 \% & Zarr Blosc(cname='blosclz', shuffle=NOSHUFFLE, blocksize=0) & 100.0 \% \\
HDF5 shuffle MAFISC-LZMA all-row-chunk & 77.7 \% & Zarr Blosc(cname='snappy', shuffle=SHUFFLE, blocksize=0) & 100.0 \% \\
LZMA LEB128S-delta-column DELTA distance-1 & 77.8 \% & Zarr Blosc(cname='snappy', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 100.0 \% \\
LZMA LEB128S-delta-column DELTA distance-2 & 78.4 \% & LZMA raw-row DELTA distance-3 & 100.0 \% \\
HDF5 no-shuffle bitshuffle-lz4 all-column-chunk & 78.7 \% & HDF5 no-shuffle ('SZIP', 'nn', 16) all-column-chunk & 100.2 \% \\
HDF5 no-shuffle bitshuffle-lz4 individual-dsets & 78.7 \% & HDF5 no-shuffle ('SZIP', 'nn', 16) individual-dsets & 100.2 \% \\
HDF5 shuffle MAFISC-LZMA all-column-chunk & 80.8 \% & HDF5 no-shuffle ('SZIP', 'nn', 2) all-column-chunk & 100.6 \% \\
LZMA LEB128S-delta-column DELTA distance-4 & 81.5 \% & HDF5 no-shuffle ('SZIP', 'nn', 2) individual-dsets & 100.6 \% \\
LZMA raw-row DELTA distance-2 & 83.2 \% & HDF5 shuffle bitshuffle-lz4 all-row-chunk & 101.2 \% \\
Zarr Blosc-zstd shuffle=NOSHUFFLE, blocksize=0) & 83.5 \% & HDF5 no-shuffle gzip all-column-chunk & 101.4 \% \\
Zarr Blosc-zstd shuffle=BITSHUFFLE, blocksize=0) & 83.5 \% & HDF5 no-shuffle gzip individual-dsets & 101.4 \% \\
LZMA LEB128S-row DELTA distance-4 & 83.9 \% & HDF5 no-shuffle ('SZIP', 'nn', 24) all-column-chunk & 102.7 \% \\
LZMA raw-row DELTA distance-4 & 84.6 \% & HDF5 no-shuffle ('SZIP', 'nn', 24) individual-dsets & 102.7 \% \\
LZMA raw-column DELTA distance-3 & 85.3 \% & ZLIB LEB128S-column & 103.1 \% \\
HDF5 shuffle lzf all-column-chunk & 85.5 \% & HDF5 no-shuffle ('SZIP', 'nn', 32) all-column-chunk & 105.0 \% \\
HDF5 shuffle lzf individual-dsets & 85.5 \% & HDF5 no-shuffle ('SZIP', 'nn', 32) individual-dsets & 105.0 \% \\
LZMA LEB128S-delta-column DELTA distance-3 & 86.8 \% & LZMA LEB128S-column DELTA distance-1 & 105.1 \% \\
HDF5 shuffle bitshuffle-lz4 all-column-chunk & 86.9 \% & HDF5 shuffle ('SZIP', 'nn', 4) all-column-chunk & 105.1 \% \\
HDF5 shuffle bitshuffle-lz4 individual-dsets & 86.9 \% & HDF5 shuffle ('SZIP', 'nn', 4) individual-dsets & 105.1 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zstd') all-column-chunk & 87.4 \% & HDF5 shuffle ('SZIP', 'nn', 8) all-column-chunk & 107.8 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zstd') all-column-chunk & 87.4 \% & HDF5 shuffle ('SZIP', 'nn', 8) individual-dsets & 107.8 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zstd') all-column-chunk & 87.4 \% & HDF5 shuffle ('SZIP', 'nn', 2) all-column-chunk & 108.4 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zstd') all-column-chunk & 87.4 \% & HDF5 shuffle ('SZIP', 'nn', 2) individual-dsets & 108.4 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zstd') all-column-chunk & 87.4 \% & LZMA LEB128S-column DELTA distance-3 & 109.3 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zstd') all-column-chunk & 87.4 \% & HDF5 shuffle lzf all-row-chunk & 109.5 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zstd') all-column-chunk & 87.4 \% & LZMA LEB128S-column DELTA distance-2 & 109.5 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zstd') all-column-chunk & 87.4 \% & HDF5 shuffle ('SZIP', 'nn', 16) all-column-chunk & 114.3 \% \\
HDF5 shuffle ('SZIP', 'nn', 16) individual-dsets & 114.3 \% & HDF5 no-shuffle lzf individual-dsets & 171.7 \% \\
LZMA LEB128S-column DELTA distance-4 & 115.3 \% & HDF5 no-shuffle ('SZIP', 'ec', 2) individual-dsets & 176.0 \% \\
HDF5 no-shuffle gzip all-row-chunk & 116.3 \% & HDF5 no-shuffle ('SZIP', 'ec', 2) all-column-chunk & 176.0 \% \\
HDF5 shuffle ('SZIP', 'nn', 24) all-column-chunk & 118.7 \% & HDF5 shuffle ('SZIP', 'ec', 2) individual-dsets & 176.7 \% \\
HDF5 shuffle ('SZIP', 'nn', 24) individual-dsets & 118.7 \% & HDF5 shuffle ('SZIP', 'ec', 2) all-column-chunk & 176.7 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4hc') all-column-chunk & 122.2 \% & HDF5 no-shuffle lzf all-row-chunk & 180.4 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4hc') all-column-chunk & 122.2 \% & HDF5 shuffle ('SZIP', 'nn', 4) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4hc') all-column-chunk & 122.2 \% & HDF5 no-shuffle ('SZIP', 'ec', 8) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4hc') all-column-chunk & 122.2 \% & HDF5 no-shuffle ('SZIP', 'nn', 16) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4hc') all-column-chunk & 122.2 \% & HDF5 no-shuffle ('SZIP', 'nn', 8) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4hc') all-column-chunk & 122.2 \% & HDF5 no-shuffle ('SZIP', 'nn', 32) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4hc') all-column-chunk & 122.2 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4hc') all-column-chunk & 122.2 \% & HDF5 no-shuffle ('SZIP', 'nn', 2) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4hc') all-column-chunk & 122.2 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'blosclz') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4hc') individual-dsets & 122.3 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'blosclz') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4hc') individual-dsets & 122.3 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'blosclz') all-column-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4hc') individual-dsets & 122.3 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4hc') individual-dsets & 122.3 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'blosclz') all-column-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4hc') individual-dsets & 122.3 \% & HDF5 no-shuffle ('SZIP', 'ec', 4) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4hc') individual-dsets & 122.3 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'blosclz') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4hc') individual-dsets & 122.3 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'blosclz') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4hc') individual-dsets & 122.3 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'blosclz') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4hc') individual-dsets & 122.3 \% & HDF5 shuffle ('SZIP', 'nn', 24) all-row-chunk & 200.0 \% \\
HDF5 shuffle ('SZIP', 'nn', 32) all-column-chunk & 122.6 \% & HDF5 shuffle ('SZIP', 'ec', 2) all-row-chunk & 200.0 \% \\
HDF5 shuffle ('SZIP', 'nn', 32) individual-dsets & 122.6 \% & HDF5 shuffle ('SZIP', 'ec', 4) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zstd') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'blosclz') all-column-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zstd') all-row-chunk & 129.8 \% & HDF5 shuffle ('SZIP', 'ec', 16) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zstd') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('SZIP', 'ec', 32) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zstd') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'blosclz') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zstd') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zstd') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'blosclz') all-column-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zstd') all-row-chunk & 129.8 \% & HDF5 shuffle ('SZIP', 'ec', 8) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zstd') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('SZIP', 'ec', 2) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zstd') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'blosclz') all-column-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zlib') all-row-chunk & 129.8 \% & HDF5 shuffle ('SZIP', 'nn', 16) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zlib') all-row-chunk & 129.8 \% & HDF5 shuffle ('SZIP', 'nn', 32) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zlib') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'blosclz') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zlib') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zlib') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'blosclz') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zlib') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('SZIP', 'ec', 24) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zlib') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('SZIP', 'ec', 16) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zlib') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('SZIP', 'nn', 24) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zlib') all-row-chunk & 129.8 \% & HDF5 shuffle ('SZIP', 'nn', 2) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'snappy') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'snappy') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'blosclz') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'snappy') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'snappy') all-row-chunk & 129.8 \% & HDF5 shuffle ('SZIP', 'ec', 24) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'snappy') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'blosclz') all-column-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'snappy') all-row-chunk & 129.8 \% & HDF5 shuffle ('SZIP', 'nn', 8) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'snappy') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('SZIP', 'nn', 4) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'snappy') all-row-chunk & 129.8 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'snappy') all-row-chunk & 129.8 \% & HDF5 shuffle ('SZIP', 'ec', 32) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4') all-column-chunk & 142.1 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'blosclz') all-column-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4') all-column-chunk & 142.1 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'blosclz') all-column-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4') all-column-chunk & 142.1 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4') all-column-chunk & 142.1 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'blosclz') all-column-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4') all-column-chunk & 142.1 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4') all-column-chunk & 142.1 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'blosclz') individual-dsets & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4') all-column-chunk & 142.1 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'blosclz') individual-dsets & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4') all-column-chunk & 142.1 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'blosclz') individual-dsets & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4') all-column-chunk & 142.1 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'blosclz') individual-dsets & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4') individual-dsets & 142.2 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'blosclz') individual-dsets & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4') individual-dsets & 142.2 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'blosclz') individual-dsets & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4') individual-dsets & 142.2 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'blosclz') individual-dsets & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4') individual-dsets & 142.2 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'blosclz') individual-dsets & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4') individual-dsets & 142.2 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'blosclz') individual-dsets & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4') individual-dsets & 142.2 \%  \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4') individual-dsets & 142.2 \%  \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4') individual-dsets & 142.2 \%  \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4') individual-dsets & 142.2 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 16) all-column-chunk & 161.4 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 16) individual-dsets & 161.4 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 24) all-column-chunk & 161.9 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 24) individual-dsets & 161.9 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 8) all-column-chunk & 161.9 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 8) individual-dsets & 161.9 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 32) all-column-chunk & 162.6 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 32) individual-dsets & 162.7 \%  \\
HDF5 shuffle ('SZIP', 'ec', 8) all-column-chunk & 164.6 \%  \\
HDF5 shuffle ('SZIP', 'ec', 8) individual-dsets & 164.6 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 4) all-column-chunk & 165.9 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 4) individual-dsets & 165.9 \%  \\
HDF5 shuffle ('SZIP', 'ec', 16) all-column-chunk & 166.0 \%  \\
HDF5 shuffle ('SZIP', 'ec', 16) individual-dsets & 166.0 \%  \\
HDF5 shuffle ('SZIP', 'ec', 4) all-column-chunk & 167.3 \%  \\
HDF5 shuffle ('SZIP', 'ec', 4) individual-dsets & 167.3 \%  \\
HDF5 shuffle ('SZIP', 'ec', 24) all-column-chunk & 168.2 \%  \\
HDF5 shuffle ('SZIP', 'ec', 24) individual-dsets & 168.2 \%  \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4hc') all-row-chunk & 168.3 \%  \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4hc') all-row-chunk & 168.3 \%  \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4hc') all-row-chunk & 168.3 \%  \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4hc') all-row-chunk & 168.3 \%  \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4hc') all-row-chunk & 168.3 \%  \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4hc') all-row-chunk & 168.3 \%  \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4hc') all-row-chunk & 168.3 \%  \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4hc') all-row-chunk & 168.3 \%  \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4hc') all-row-chunk & 168.3 \%  \\
HDF5 shuffle ('SZIP', 'ec', 32) all-column-chunk & 170.6 \%  \\
HDF5 shuffle ('SZIP', 'ec', 32) individual-dsets & 170.6 \%  \\
HDF5 no-shuffle lzf all-column-chunk & 171.7 \%  \\
\end{longtable}
\tiny \begin{longtable}{lc|lc}
\caption{BLOND-250: Data representation benchmark \numberOfDataRepresentations{} formats and data transformations. Raw input data size was \SI{11898.9}{\gibi\byte} from 35490 files.} \\
\textbf{Name} & \textbf{Compression Ratio} & \textbf{Name} & \textbf{Compression Ratio} \\ \hline \endhead
ALAC PCM-16 & 44.6 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zstd') individual-dsets & 78.2 \% \\
HDF5 no-shuffle MAFISC-LZMA all-column-chunk & 45.9 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zstd') individual-dsets & 78.2 \% \\
LZMA-alone LEB128S-delta-row & 48.8 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zstd') individual-dsets & 78.2 \% \\
LZMA-xz LEB128S-delta-row & 48.8 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zstd') individual-dsets & 78.2 \% \\
Zarr BZ2 (Delta(dtype='<i2'),) & 49.0 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zstd') individual-dsets & 78.2 \% \\
bzip2 LEB128S-delta-row & 49.7 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zstd') individual-dsets & 78.2 \% \\
Zarr LZMA (Delta(dtype='<i2'),) & 51.4 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zstd') individual-dsets & 78.2 \% \\
zstd-22 LEB128S-delta-row & 51.8 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zstd') individual-dsets & 78.2 \% \\
FLAC PCM-16 & 51.8 \% & HDF5 no-shuffle ('SZIP', 'nn', 8) all-column-chunk & 78.2 \% \\
WavPack PCM-16 & 51.9 \% & HDF5 no-shuffle ('SZIP', 'nn', 8) individual-dsets & 78.3 \% \\
LZMA raw-column DELTA distance-2 & 51.9 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zlib') all-column-chunk & 78.8 \% \\
Zarr Blosc(cname='zlib', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 52.1 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zlib') all-column-chunk & 78.8 \% \\
Zarr Blosc-zstd shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 52.4 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zlib') all-column-chunk & 78.8 \% \\
LZMA raw-column DELTA distance-4 & 52.7 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zlib') all-column-chunk & 78.8 \% \\
HDF5 shuffle zstd individual-dsets & 52.8 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zlib') all-column-chunk & 78.8 \% \\
HDF5 shuffle zstd all-column-chunk & 53.0 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zlib') all-column-chunk & 78.8 \% \\
LZMA-alone LEB128S-delta-column & 53.1 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zlib') all-column-chunk & 78.8 \% \\
LZMA-xz LEB128S-delta-column & 53.1 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zlib') all-column-chunk & 78.8 \% \\
Zarr Blosc(cname='lz4hc', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 53.8 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zlib') all-column-chunk & 78.8 \% \\
Zarr Blosc(cname='zlib', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 53.9 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zlib') individual-dsets & 78.8 \% \\
LZMA-alone raw-column & 54.8 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zlib') individual-dsets & 78.8 \% \\
LZMA-xz raw-column & 54.8 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zlib') individual-dsets & 78.8 \% \\
Zarr Blosc(cname='lz4', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 55.4 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zlib') individual-dsets & 78.8 \% \\
Zarr Blosc-zstd shuffle=SHUFFLE, blocksize=0) & 55.5 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zlib') individual-dsets & 78.8 \% \\
bzip2 LEB128S-delta-column & 55.8 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zlib') individual-dsets & 78.8 \% \\
zstd-22 LEB128S-delta-column & 55.9 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zlib') individual-dsets & 78.8 \% \\
LZMA-alone LEB128S-row & 55.9 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zlib') individual-dsets & 78.8 \% \\
LZMA-xz LEB128S-row & 55.9 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zlib') individual-dsets & 78.8 \% \\
LZMA raw-column DELTA distance-1 & 56.5 \% & LZMA raw-row DELTA distance-2 & 79.3 \% \\
LZMA LEB128S-delta-row DELTA distance-1 & 56.6 \% & HDF5 no-shuffle ('SZIP', 'nn', 16) all-column-chunk & 79.9 \% \\
ZLIB LEB128S-delta-row & 56.8 \% & HDF5 no-shuffle ('SZIP', 'nn', 16) individual-dsets & 79.9 \% \\
LZMA LEB128S-delta-row DELTA distance-2 & 57.1 \% & Zarr Blosc-zstd shuffle=NOSHUFFLE, blocksize=0) & 80.1 \% \\
Zarr Blosc-zstd shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 57.9 \% & Zarr Blosc-zstd shuffle=BITSHUFFLE, blocksize=0) & 80.1 \% \\
Zarr Blosc-zstd shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 57.9 \% & LZMA raw-row DELTA distance-4 & 80.3 \% \\
Zarr Blosc(cname='zlib', shuffle=BITSHUFFLE, blocksize=0) & 58.2 \% & Zarr Blosc(cname='snappy', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 80.7 \% \\
Zarr Blosc(cname='zlib', shuffle=SHUFFLE, blocksize=0) & 58.2 \% & Zarr Blosc(cname='lz4hc', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 81.0 \% \\
Zarr Blosc(cname='blosclz', shuffle=BITSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 58.4 \% & HDF5 no-shuffle ('SZIP', 'nn', 24) all-column-chunk & 81.2 \% \\
LZMA LEB128S-delta-row DELTA distance-4 & 58.7 \% & HDF5 no-shuffle ('SZIP', 'nn', 24) individual-dsets & 81.3 \% \\
Zarr LZMA & 59.3 \% & HDF5 no-shuffle ('SZIP', 'nn', 2) all-column-chunk & 81.3 \% \\
HDF5 shuffle gzip all-column-chunk & 59.7 \% & HDF5 no-shuffle ('SZIP', 'nn', 2) individual-dsets & 81.3 \% \\
HDF5 shuffle gzip individual-dsets & 59.7 \% & HDF5 no-shuffle ('SZIP', 'nn', 32) all-column-chunk & 82.6 \% \\
ZLIB LEB128S-delta-column & 59.8 \% & HDF5 no-shuffle ('SZIP', 'nn', 32) individual-dsets & 82.6 \% \\
HDF5 shuffle zstd all-row-chunk & 59.9 \% & HDF5 no-shuffle bitshuffle-lz4 all-row-chunk & 84.8 \% \\
Zarr Blosc(cname='lz4hc', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 60.3 \% & HDF5 shuffle ('SZIP', 'nn', 8) all-column-chunk & 85.0 \% \\
LZMA LEB128S-delta-row DELTA distance-3 & 60.4 \% & HDF5 shuffle ('SZIP', 'nn', 8) individual-dsets & 85.0 \% \\
LZMA LEB128S-delta-column DELTA distance-1 & 61.0 \% & HDF5 shuffle ('SZIP', 'nn', 4) all-column-chunk & 85.1 \% \\
HDF5 no-shuffle MAFISC-LZMA individual-dsets & 61.2 \% & HDF5 shuffle ('SZIP', 'nn', 4) individual-dsets & 85.1 \% \\
Zarr Blosc(cname='lz4hc', shuffle=SHUFFLE, blocksize=0) & 61.7 \% & HDF5 no-shuffle gzip all-column-chunk & 86.4 \% \\
Zarr Blosc(cname='lz4hc', shuffle=BITSHUFFLE, blocksize=0) & 62.1 \% & HDF5 no-shuffle gzip individual-dsets & 86.4 \% \\
HDF5 no-shuffle zstd individual-dsets & 62.4 \% & HDF5 shuffle bitshuffle-lz4 all-row-chunk & 86.5 \% \\
HDF5 no-shuffle zstd all-column-chunk & 62.6 \% & zstd-22 raw-row & 86.9 \% \\
Zarr Zlib(level=9) (Delta(dtype='<i2'),) & 62.6 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'snappy') all-column-chunk & 87.3 \% \\
LZMA LEB128S-delta-column DELTA distance-2 & 62.7 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'snappy') all-column-chunk & 87.3 \% \\
bzip2 raw-column & 62.8 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'snappy') all-column-chunk & 87.3 \% \\
bzip2 LEB128S-row & 63.3 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'snappy') all-column-chunk & 87.3 \% \\
Zarr BZ2 & 63.5 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'snappy') all-column-chunk & 87.3 \% \\
Zarr Blosc(cname='zlib', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 63.5 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'snappy') all-column-chunk & 87.3 \% \\
LZMA LEB128S-delta-column DELTA distance-3 & 64.0 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'snappy') all-column-chunk & 87.3 \% \\
LZMA LEB128S-delta-column DELTA distance-4 & 64.5 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'snappy') all-column-chunk & 87.3 \% \\
Zarr Blosc(cname='lz4', shuffle=BITSHUFFLE, blocksize=0) & 65.8 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'snappy') all-column-chunk & 87.3 \% \\
zstd-22 raw-column & 66.0 \% & Zarr Blosc(cname='lz4', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 87.3 \% \\
HDF5 no-shuffle MAFISC-LZMA all-row-chunk & 66.1 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'snappy') individual-dsets & 87.3 \% \\
HDF5 shuffle gzip all-row-chunk & 66.4 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'snappy') individual-dsets & 87.3 \% \\
HDF5 shuffle MAFISC-LZMA individual-dsets & 66.4 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'snappy') individual-dsets & 87.3 \% \\
HDF5 no-shuffle zstd all-row-chunk & 66.6 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'snappy') individual-dsets & 87.3 \% \\
LZMA LEB128S-row DELTA distance-2 & 66.9 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'snappy') individual-dsets & 87.3 \% \\
zstd-22 LEB128S-row & 66.9 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'snappy') individual-dsets & 87.3 \% \\
Zarr Blosc(cname='blosclz', shuffle=BITSHUFFLE, blocksize=0) & 67.2 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'snappy') individual-dsets & 87.3 \% \\
Zarr Blosc(cname='blosclz', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 68.1 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'snappy') individual-dsets & 87.3 \% \\
LZMA LEB128S-row DELTA distance-3 & 68.5 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'snappy') individual-dsets & 87.3 \% \\
HDF5 no-shuffle bitshuffle-lz4 all-column-chunk & 68.6 \% & ZLIB raw-column & 87.5 \% \\
HDF5 no-shuffle bitshuffle-lz4 individual-dsets & 68.6 \% & Zarr Zlib(level=9) & 87.5 \% \\
LZMA LEB128S-row DELTA distance-1 & 68.7 \% & Zarr Blosc(cname='zlib', shuffle=NOSHUFFLE, blocksize=0) & 87.6 \% \\
HDF5 shuffle MAFISC-LZMA all-row-chunk & 69.2 \% & HDF5 shuffle ('SZIP', 'nn', 16) all-column-chunk & 88.2 \% \\
Zarr Blosc(cname='lz4', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 69.8 \% & HDF5 shuffle ('SZIP', 'nn', 16) individual-dsets & 88.2 \% \\
LZMA-alone raw-row & 70.0 \% & Zarr Blosc(cname='snappy', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 89.1 \% \\
LZMA-xz raw-row & 70.0 \% & HDF5 shuffle ('SZIP', 'nn', 2) all-column-chunk & 90.6 \% \\
LZMA-alone LEB128S-column & 70.8 \% & HDF5 shuffle ('SZIP', 'nn', 2) individual-dsets & 90.6 \% \\
LZMA-xz LEB128S-column & 70.8 \% & zstd-22 LEB128S-column & 91.0 \% \\
HDF5 shuffle MAFISC-LZMA all-column-chunk & 71.0 \% & HDF5 shuffle ('SZIP', 'nn', 24) all-column-chunk & 91.1 \% \\
Zarr Blosc(cname='lz4', shuffle=SHUFFLE, blocksize=0) & 71.7 \% & HDF5 shuffle ('SZIP', 'nn', 24) individual-dsets & 91.1 \% \\
Zarr Blosc(cname='blosclz', shuffle=SHUFFLE, blocksize=0) & 71.9 \% & HDF5 shuffle lzf all-row-chunk & 92.0 \% \\
LZMA LEB128S-row DELTA distance-4 & 74.7 \% & ZLIB raw-row & 92.2 \% \\
LZMA raw-column DELTA distance-3 & 75.8 \% & bzip2 raw-row & 92.6 \% \\
HDF5 shuffle bitshuffle-lz4 all-column-chunk & 76.5 \% & LZMA raw-row DELTA distance-1 & 93.0 \% \\
HDF5 shuffle bitshuffle-lz4 individual-dsets & 76.5 \% & Zarr Blosc(cname='blosclz', shuffle=NOSHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 93.2 \% \\
HDF5 shuffle lzf all-column-chunk & 77.7 \% & ZLIB LEB128S-row & 93.4 \% \\
HDF5 shuffle lzf individual-dsets & 77.7 \% & HDF5 shuffle ('SZIP', 'nn', 32) all-column-chunk & 93.7 \% \\
HDF5 no-shuffle ('SZIP', 'nn', 4) all-column-chunk & 77.9 \% & HDF5 shuffle ('SZIP', 'nn', 32) individual-dsets & 93.7 \% \\
HDF5 no-shuffle ('SZIP', 'nn', 4) individual-dsets & 77.9 \% & bzip2 LEB128S-column & 94.7 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zstd') all-column-chunk & 78.2 \% & Zarr Blosc(cname='lz4hc', shuffle=NOSHUFFLE, blocksize=0) & 98.4 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zstd') all-column-chunk & 78.2 \% & Zarr Blosc(cname='snappy', shuffle=BITSHUFFLE, blocksize=0) & 99.5 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zstd') all-column-chunk & 78.2 \% & Zarr Blosc(cname='lz4', shuffle=NOSHUFFLE, blocksize=0) & 99.8 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zstd') all-column-chunk & 78.2 \% & Zarr Blosc(cname='snappy', shuffle=NOSHUFFLE, blocksize=0) & 100.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zstd') all-column-chunk & 78.2 \% & Zarr None & 100.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zstd') all-column-chunk & 78.2 \% & Zarr None (Delta(dtype='<i2'),) & 100.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zstd') all-column-chunk & 78.2 \% & RAW-UNCOMPRESSED & 100.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zstd') all-column-chunk & 78.2 \% & Zarr Blosc(cname='blosclz', shuffle=NOSHUFFLE, blocksize=0) & 100.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zstd') all-column-chunk & 78.2 \% & Zarr Blosc(cname='snappy', shuffle=SHUFFLE, blocksize=0) & 100.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zstd') individual-dsets & 78.2 \% & Zarr Blosc(cname='snappy', shuffle=SHUFFLE, blocksize=0) (Delta(dtype='<i2'),) & 100.0 \% \\
LZMA raw-row DELTA distance-3 & 100.0 \% & HDF5 no-shuffle lzf individual-dsets & 167.9 \% \\
ZLIB LEB128S-column & 100.9 \% & HDF5 no-shuffle ('SZIP', 'ec', 2) all-column-chunk & 170.8 \% \\
LZMA LEB128S-column DELTA distance-1 & 103.1 \% & HDF5 no-shuffle ('SZIP', 'ec', 2) individual-dsets & 170.8 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4hc') all-column-chunk & 106.4 \% & HDF5 shuffle ('SZIP', 'ec', 2) all-column-chunk & 172.6 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4hc') all-column-chunk & 106.4 \% & HDF5 shuffle ('SZIP', 'ec', 2) individual-dsets & 172.6 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4hc') all-column-chunk & 106.4 \% & HDF5 no-shuffle lzf all-row-chunk & 173.6 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4hc') all-column-chunk & 106.4 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4') all-row-chunk & 199.8 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4hc') all-column-chunk & 106.4 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4') all-row-chunk & 199.8 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4hc') all-column-chunk & 106.4 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4') all-row-chunk & 199.8 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4hc') all-column-chunk & 106.4 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4') all-row-chunk & 199.8 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4hc') all-column-chunk & 106.4 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4') all-row-chunk & 199.8 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4hc') all-column-chunk & 106.4 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4') all-row-chunk & 199.8 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4hc') individual-dsets & 106.4 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4') all-row-chunk & 199.8 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4hc') individual-dsets & 106.4 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4') all-row-chunk & 199.8 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4hc') individual-dsets & 106.4 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4') all-row-chunk & 199.8 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4hc') individual-dsets & 106.4 \% & HDF5 shuffle ('SZIP', 'nn', 4) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4hc') individual-dsets & 106.4 \% & HDF5 no-shuffle ('SZIP', 'ec', 8) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4hc') individual-dsets & 106.4 \% & HDF5 no-shuffle ('SZIP', 'nn', 16) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4hc') individual-dsets & 106.4 \% & HDF5 no-shuffle ('SZIP', 'nn', 8) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4hc') individual-dsets & 106.4 \% & HDF5 no-shuffle ('SZIP', 'nn', 32) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4hc') individual-dsets & 106.4 \% & HDF5 no-shuffle ('SZIP', 'nn', 2) all-row-chunk & 200.0 \% \\
LZMA LEB128S-column DELTA distance-3 & 106.6 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'blosclz') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle gzip all-row-chunk & 106.7 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'blosclz') all-row-chunk & 200.0 \% \\
LZMA LEB128S-column DELTA distance-2 & 106.7 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'blosclz') all-column-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zstd') all-row-chunk & 107.5 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'blosclz') all-column-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zstd') all-row-chunk & 107.5 \% & HDF5 no-shuffle ('SZIP', 'ec', 4) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zstd') all-row-chunk & 107.5 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'blosclz') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zstd') all-row-chunk & 107.5 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'blosclz') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zstd') all-row-chunk & 107.5 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'blosclz') all-column-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zstd') all-row-chunk & 107.5 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'blosclz') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zstd') all-row-chunk & 107.5 \% & HDF5 shuffle ('SZIP', 'nn', 24) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zstd') all-row-chunk & 107.5 \% & HDF5 shuffle ('SZIP', 'ec', 2) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zstd') all-row-chunk & 107.5 \% & HDF5 shuffle ('SZIP', 'ec', 8) all-row-chunk & 200.0 \% \\
LZMA LEB128S-column DELTA distance-4 & 111.9 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'blosclz') all-column-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'snappy') all-row-chunk & 120.3 \% & HDF5 shuffle ('SZIP', 'ec', 16) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'zlib') all-row-chunk & 120.3 \% & HDF5 no-shuffle ('SZIP', 'ec', 32) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'snappy') all-row-chunk & 120.3 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'blosclz') all-column-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'snappy') all-row-chunk & 120.3 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'blosclz') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'zlib') all-row-chunk & 120.3 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'blosclz') all-column-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'zlib') all-row-chunk & 120.3 \% & HDF5 no-shuffle ('SZIP', 'ec', 2) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'snappy') all-row-chunk & 120.3 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'blosclz') all-column-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'zlib') all-row-chunk & 120.3 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'blosclz') all-column-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'zlib') all-row-chunk & 120.3 \% & HDF5 shuffle ('SZIP', 'nn', 16) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'snappy') all-row-chunk & 120.3 \% & HDF5 shuffle ('SZIP', 'nn', 32) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'zlib') all-row-chunk & 120.3 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'blosclz') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'zlib') all-row-chunk & 120.3 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'blosclz') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'zlib') all-row-chunk & 120.3 \% & HDF5 no-shuffle ('SZIP', 'ec', 24) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'snappy') all-row-chunk & 120.3 \% & HDF5 no-shuffle ('SZIP', 'ec', 16) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'snappy') all-row-chunk & 120.3 \% & HDF5 no-shuffle ('SZIP', 'nn', 24) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'snappy') all-row-chunk & 120.3 \% & HDF5 shuffle ('SZIP', 'nn', 2) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'snappy') all-row-chunk & 120.3 \% & HDF5 shuffle ('SZIP', 'ec', 4) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'zlib') all-row-chunk & 120.3 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'blosclz') all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4hc') all-row-chunk & 120.7 \% & HDF5 shuffle ('SZIP', 'ec', 24) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4hc') all-row-chunk & 120.7 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'blosclz') all-column-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4hc') all-row-chunk & 120.7 \% & HDF5 shuffle ('SZIP', 'nn', 8) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4hc') all-row-chunk & 120.7 \% & HDF5 no-shuffle ('SZIP', 'nn', 4) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4hc') all-row-chunk & 120.7 \% & HDF5 shuffle ('SZIP', 'ec', 32) all-row-chunk & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4hc') all-row-chunk & 120.7 \% & HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'blosclz') individual-dsets & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4hc') all-row-chunk & 120.7 \% & HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'blosclz') individual-dsets & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4hc') all-row-chunk & 120.7 \% & HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'blosclz') individual-dsets & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4hc') all-row-chunk & 120.7 \% & HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'blosclz') individual-dsets & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4') individual-dsets & 130.0 \% & HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'blosclz') individual-dsets & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4') individual-dsets & 130.0 \% & HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'blosclz') individual-dsets & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4') individual-dsets & 130.0 \% & HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'blosclz') individual-dsets & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4') individual-dsets & 130.0 \% & HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'blosclz') individual-dsets & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4') individual-dsets & 130.0 \% & HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'blosclz') individual-dsets & 200.0 \% \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4') individual-dsets & 130.0 \%  \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4') individual-dsets & 130.0 \%  \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4') individual-dsets & 130.0 \%  \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4') individual-dsets & 130.0 \%  \\
HDF5 no-shuffle ('Blosc', 3, 'SHUFFLE', 'lz4') all-column-chunk & 130.0 \%  \\
HDF5 no-shuffle ('Blosc', 8, 'SHUFFLE', 'lz4') all-column-chunk & 130.0 \%  \\
HDF5 no-shuffle ('Blosc', 4, 'BITSHUFFLE', 'lz4') all-column-chunk & 130.0 \%  \\
HDF5 no-shuffle ('Blosc', 8, 'NOSHUFFLE', 'lz4') all-column-chunk & 130.0 \%  \\
HDF5 no-shuffle ('Blosc', 3, 'BITSHUFFLE', 'lz4') all-column-chunk & 130.0 \%  \\
HDF5 no-shuffle ('Blosc', 3, 'NOSHUFFLE', 'lz4') all-column-chunk & 130.0 \%  \\
HDF5 no-shuffle ('Blosc', 4, 'SHUFFLE', 'lz4') all-column-chunk & 130.0 \%  \\
HDF5 no-shuffle ('Blosc', 4, 'NOSHUFFLE', 'lz4') all-column-chunk & 130.0 \%  \\
HDF5 no-shuffle ('Blosc', 8, 'BITSHUFFLE', 'lz4') all-column-chunk & 130.0 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 24) all-column-chunk & 153.3 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 24) individual-dsets & 153.3 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 16) all-column-chunk & 153.5 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 16) individual-dsets & 153.5 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 32) all-column-chunk & 153.6 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 32) individual-dsets & 153.6 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 8) all-column-chunk & 155.2 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 8) individual-dsets & 155.2 \%  \\
HDF5 shuffle ('SZIP', 'ec', 16) all-column-chunk & 155.8 \%  \\
HDF5 shuffle ('SZIP', 'ec', 16) individual-dsets & 155.8 \%  \\
HDF5 shuffle ('SZIP', 'ec', 24) all-column-chunk & 156.5 \%  \\
HDF5 shuffle ('SZIP', 'ec', 24) individual-dsets & 156.5 \%  \\
HDF5 shuffle ('SZIP', 'ec', 8) all-column-chunk & 156.6 \%  \\
HDF5 shuffle ('SZIP', 'ec', 8) individual-dsets & 156.6 \%  \\
HDF5 shuffle ('SZIP', 'ec', 32) all-column-chunk & 157.4 \%  \\
HDF5 shuffle ('SZIP', 'ec', 32) individual-dsets & 157.4 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 4) all-column-chunk & 159.7 \%  \\
HDF5 no-shuffle ('SZIP', 'ec', 4) individual-dsets & 159.7 \%  \\
HDF5 shuffle ('SZIP', 'ec', 4) all-column-chunk & 161.3 \%  \\
HDF5 shuffle ('SZIP', 'ec', 4) individual-dsets & 161.3 \%  \\
HDF5 no-shuffle lzf all-column-chunk & 167.9 \%  \\
\end{longtable}

